Count-Min Sketch with Conservative Updates: Worst-Case Analysis

Count-Min Sketch with Conservative Updates (CMS-CU) is a memory-efficient hash-based data structure used to estimate the occurrences of items within a data stream. CMS-CU stores $m$ counters and employs $d$ hash functions to map items to these counters. We first argue that the estimation error in CMS-CU is maximal when each item appears at most once in the stream. Next, we study CMS-CU in this setting. In the case where $d=m-1$, we prove that the average estimation error and the average counter rate converge almost surely to $\frac{1}{2}$, contrasting with the vanilla Count-Min Sketch, where the average counter rate is equal to $\frac{m-1}{m}$. For any given $m$ and $d$, we prove novel lower and upper bounds on the average estimation error, incorporating a positive integer parameter $g$. Larger values of this parameter improve the accuracy of the bounds. Moreover, the computation of each bound involves examining an ergodic Markov process with a state space of size $\binom{m+g-d}{g}$ and a sparse transition probabilities matrix containing $\mathcal{O}(m\binom{m+g-d}{g})$ non-zero entries. For $d=m-1$, $g=1$, and as $m\to \infty$, we show that the lower and upper bounds coincide. In general, our bounds exhibit high accuracy for small values of $g$, as shown by numerical computation. For example, for $m=50$, $d=4$, and $g=5$, the difference between the lower and upper bounds is smaller than $10^{-4}$.

==> Introductions/introduction_09April.tex <==
Counting occurrences and determining the most prevalent items within a data stream represents a fundamental challenge~\cite{baryossef2002couting, CHARIKAR2004CountSketch, cormode2005improved}. The task of counting and estimating frequencies holds significance across a spectrum of fields, spanning from network traffic surveillance to click stream analytics, content delivery networks, predictive maintenance, and fraud detection~\cite{nelson2012sketching, Basat2021Salsa, AnomalyDetectionCMS2021, TinyLFU2017}. 

Although the concept of counting may appear straightforward initially---simply incrementing a counter upon encountering an item---the reality is far more complex, especially when confronted with the deluge of real-time data streams characteristic of many practical applications. As data volumes surge, maintaining a dedicated counter for each potential item within costly, high-speed storage becomes unfeasible~\cite{ankleshwaria2014mining}. 

Due to the practical non feasibility of exact counting, many applications rely on approximate counting algorithms. These algorithms leverage probabilistic data structures such as %\texttt{HyperLogLog}~\cite{flajolet2007hyperloglog},
\emph{Spectral Bloom Filters} (\texttt{SBF})~\cite{SpectralBloomFilters2003}, \emph{Count-Sketch} (\texttt{CS})~\cite{CHARIKAR2004CountSketch}, \emph{Count-Min Sketch} (\texttt{CMS})~\cite{cormode2005improved}, and \emph{Count-Min Sketch with Conservative Updates} (\texttt{CMS-CU})~\cite{ConservativeUpdate2002}, which sacrifice perfect accuracy for scalability and efficiency in handling massive data streams. 

% \texttt{SBF} uses hash functions to map elements to a bit array for membership queries. \texttt{HyperLogLog} analyzes leading zeros in hashes to estimate cardinality. \texttt{CS} combines hash functions and a hash table for frequency estimation with positive and negative updates. \texttt{CMS} and \texttt{CMS-CU} both estimate element frequencies with a two-dimensional array of counters and hash functions, with \texttt{CMS-CU} implementing a conservative update (a.k.a. Minimal Increment~\cite{SpectralBloomFilters2003}), which reduces estimation errors by only incrementing counters without decrementing them, thus enhancing accuracy compared to \texttt{CMS}.

\texttt{CMS} comprises a matrix of counters indexed by multiple hash functions. In the vanilla \texttt{CMS} algorithm, updates involve incrementing counters corresponding to the hashed values of input items. Each item is hashed using multiple functions, incrementing counters at those positions to indicate its presence. Due to potential collisions, some counters may be incremented more often, leading to underestimation of certain frequencies. The conservative variant, \texttt{CMS-CU}, limits overestimation by comparing stored counts with proposed updates before incrementing, ensuring accurate frequency estimation while minimizing underestimation risk.

The tradeoff between the memory cost and the accuracy of vanilla \texttt{CMS} and \texttt{SBF} is well understood under different assumptions on the data stream~\cite{cormode2005improved, CormodeZipfErrorCMS2005}. This trade-off is quantified by probabilistic bounds on the estimation error, given in terms of the dimension of the counters matrix. Although conservative updates are a minor modification to \texttt{CMS}, similar theoretical bounds are lacking in the context of \texttt{CMS-CU}, because of the considerable intricacy inherent in its modeling. Analytical challenges arise from the fact that, under the conservative update rule, the update of a counter selected by a hash function is contingent upon the status of the remaining chosen counters; essentially, counters do not increment independently but rather in a closely interrelated manner.

To cope with this difficulty, simplifying assumptions are made~\cite{bianchi2012modelingCMSCU, GILBloomCMSCU}. Notably,~\cite{bianchi2012modelingCMSCU} assumes a uniform load across counters, and provides empirical evidence that the approximation error under this assumption acts as an upper bound for skewed distributions. Consequently, quantifying the approximation error under uniform load establishes general bounds for \texttt{CMS-CU}. \emph{Our paper's first contribution lies in offering theoretical support for this assertion}.
Our theoretical results in Section~\ref{sec:main_assumption} suggest that selecting counters uniformly at random at each time step within  \texttt{CMS} and \texttt{CMS-CU} maximizes the expected error for infrequent item. We conjecture that this result holds in general, and we leave the proof for a future work. 
% In particular,  we prove that selecting counters uniformly at random at each time step within \texttt{CMS} maximizes the expected error for infrequent items, and we conjecture that a similar result holds for \texttt{CMS-CU}.

\emph{Second, we prove new lower and upper bounds on the approximation error of \texttt{CMS-CU} under the uniform load assumption.}
The update process of \texttt{CMS-CU} under the balanced assumption is a Markovian Process, with an exponentially growing state space. This expansive state space limits the applicability of standard Markovian analysis techniques. To deal with the growing state space, we introduce \texttt{CU-LB} (Algorithm~\ref{alg:LB-CBF-CU}) and \texttt{CU-UB} (Algorithm~\ref{alg:LB-CBF-CU}); two variants of \texttt{CMS-CU} where the \emph{counters gap}, i.e., the difference between the values of the maximal and minimal counter, is capped by a constant $g\in\mathbb{N}$. 
% TODO: Outline of the proof
% 1. The error of CMS-CU is bounded by the errors of \texttt{CU-UB} and \texttt{CU-LB}
% 2. 



The remainder of this paper is organized as follows. 


\begin{remark}
    This instance of \texttt{CMS-CU} poses an intriguing probability problem, resembling a variation of the balls and bins load balancing problem~\cite{berenbrink2000balanced}. Specifically, the scenario involves~$m$ bins and~$n$ balls. During each time step, a ball randomly selects~$d$ bins, and it is then placed in the least loaded bin among the chosen ones. This process shares similarities with \texttt{CMS-CU} with uniform counter selection, where the bins serve as counters. The key distinction lies in the balls-into-bins variant, where at each time step, exactly one counter is incremented, in contrast to potentially incrementing up to~$d$ counters in \texttt{CMS-CU}. Exploring the connection between these problems might unveil efficient methods for computing the maximal error in \texttt{CMS-CU}.
\end{remark}


==> Introductions/introduction_14April.tex <==

Counting occurrences and determining the most prevalent items within a data stream represents a fundamental challenge~\cite{Basat2021Salsa, CHARIKAR2004CountSketch, cormode2005improved}. The task of estimating frequencies holds significance across a spectrum of fields, including network traffic monitoring~\cite{Basat2021Salsa}, content delivery networks~\cite{TinyLFU2017}, anomaly detection~\cite{AnomalyDetectionCMS2021}, and natural language processing~\cite{NLPSketchesApp2012}. 

Although the concept of counting may appear straightforward initially---simply incrementing a counter upon encountering an item---the reality is far more complex, especially when confronted with the influx of real-time data streams characteristic of many practical applications. As data volumes surge, maintaining a dedicated counter for each potential item within costly, high-speed storage becomes unfeasible~\cite{ankleshwaria2014mining}. 

Given the impracticality of exact counting, many applications turn to approximate counting algorithms to handle massive data streams efficiently, sacrificing perfect accuracy for scalability. \textit{Count-Min Sketch} ($\CMS$)~\cite{cormode2005improved} is a standout among these algorithms, widely adopted for frequency estimation due to its simplicity and effectiveness~\cite{NLPSketchesApp2012,AnomalyDetectionCMS2021,CMSApplicationEngeneiring}. Indeed, its implementation in the popular data processing library DataSketches underscores its importance in the field~\cite{cormode2020smallBook}. While numerous approximate counting algorithms have been proposed, a considerable portion of them leverage $\CMS$ as a foundational component, augmenting its capabilities with additional techniques~\cite{DiamondSketch2019,HeavyKeeper2019,hsu2019learningCM}.

$\CMS$~\cite{cormode2005improved} stores a matrix of~$m$ counters organized in~$d$ rows, where each row is indexed by a dedicated hash function. In the vanilla $\CMS$ algorithm, updates involve incrementing the~$d$ counters corresponding to the hashed values of each input item from the stream. When queried for an item's count, the sketch performs lookups by hashing elements and retrieving the minimum value among the counters.
This approach results in an overestimation error since multiple items can potentially increment the same counter.
A similar algorithm to $\CMS$ is \textit{Spectral Bloom Filter}~\cite{SpectralBloomFilters2003}, in which the $m$ counters are organized in a single row indexed by $d$ hash functions. Since counter updates in $\texttt{SBF}$ mirror those in $\CMS$, error analysis for both algorithms often relies on similar methodologies. This work studies $\texttt{SBF}$ but will keep the term $\CMS$ as more common in the literature.

$\CMS$ supports negative increments as long as the counter values remain non-negative. When increments are positive, a simple modification to $\CMS$ leads to better accuracy in frequency estimation. This modification, known as \textit{conservative update}~\cite{ConservativeUpdate2002}, avoids unnecessary increments by first comparing stored counts for an item and then only incrementing the smallest ones. The scenario of positive updates finds practical applications in caching~\cite{TinyLFU2017}, natural language processing~\cite{NLPSketchesApp2012}, and bioinformatics~\cite{CMSCUApplicationBiology2022}. 

The tradeoff between the memory cost and the accuracy of the vanilla $\CMS$ is well understood under different assumptions on the data stream~\cite{cormode2005improved, CormodeZipfErrorCMS2005}. This trade-off is quantified by probabilistic bounds on the estimation error, given in terms of the dimension of the counters matrix. Although conservative updates are a minor modification to $\CMS$, a theoretical understanding of its advantages is lacking, because of the considerable intricacy inherent in its modeling. Analytical challenges arise from the fact that, under the conservative update rule, the update of a counter selected by a hash function is contingent upon the status of the remaining chosen counters; essentially, counters do not increment independently but rather in a closely interrelated manner. 



\subsection{Related work}
Four works~\cite{bianchi2012modelingCMSCU,GILBloomCMSCU,MAZZIANE2022CMSCU,fusy2023phase} explored the advantages of the conservative variant of $\CMS$. Among these, \cite{GILBloomCMSCU, MAZZIANE2022CMSCU,fusy2023phase} assume that the data stream is a stochastic stationary process and propose probabilistic bounds on the error in terms of items' probabilities of appearing. However, the proposed bounds do not fully capture the advantages of conservative updates for items with small probabilities. Quantifying the error for such items is crucial, as empirical findings suggest that they experience larger errors compared to items with higher probabilities~\cite{bianchi2012modelingCMSCU,MAZZIANE2022CMSCU}. Further details about the studies~\cite{GILBloomCMSCU,MAZZIANE2022CMSCU,fusy2023phase} are provided in Section~\ref{sec:related}. 




 % show that when items are uniformly sampled at random from a universe of size~$n$, provided that  The papers propose probabilistic bounds on the error in terms of the items' probabilities.


Bianchi et al.~\cite{bianchi2012modelingCMSCU} diverges from~\cite{GILBloomCMSCU,MAZZIANE2022CMSCU,fusy2023phase} by considering specific counters growth in $\CMSCU$. Indeed, they examine $\CMSCU$ when at each step, $d$ counters are selected uniformly at random, instead of being chosen based on the hash values of an item in the stream. The motivation for studying $\CMSCU$ under this particular assumption is empirical evidence indicating that the estimation error for non-frequent items is maximal in this setting. Bianchi et al.~\cite{bianchi2012modelingCMSCU} approximate the dynamics of $\CMSCU$ under the uniform counters selection assumption via a \textit{fluid limit}. However, this approximation lacks theoretical justification and requires recursively solving a system of ordinary differential equations.



The $\CMSCU$ instance examined in~\cite{bianchi2012modelingCMSCU} presents an intriguing probabilistic model reminiscent of the classic \textit{balls in bins with Power of d} (\texttt{Pod}) scheme~\cite{berenbrink2000balanced}. In this paradigm, at each step, $d$ bins are randomly chosen, and a ball is then placed in one of the least loaded bins---the bins with the smallest number of balls---among the selected ones. Viewing $\CMSCU$ as a modification of this classical scheme, it places a ball in \textbf{every} bin with minimal load among the selected ones.



Both $\CMSCU$, with uniform counters selection, and \texttt{Pod} exhibit Markovian processes with an exponentially growing state space. However, a notable distinction arises in their operational dynamics. In \texttt{Pod}, each step consistently involves a single increment or ball insertion. Conversely, the number of increments per step in $\CMSCU$ is stochastic and fluctuates between $1$ and $d$, contingent upon the values of the counters at that particular step. Consequently, after $T$ rounds, the average counter value in \texttt{Pod} is exactly $T/m$, whereas, in $\CMSCU$, it spans a range between $T/m$ and $Td/m$. This variability within $\CMSCU$ complicates the computation of the average counter value, especially because of the expansive state space of the underlying Markov process. Furthermore, the computation of the approximate counting error poses additional challenges.





% Both $\CMSCU$, under the uniform counters selection, and \texttt{Pod} are Markovian Processes, with an exponentially growing state space. However, in \texttt{Pod}, each step involves a consistent number of increments, or ball insertions, always equal to~$1$, while in $\CMSCU$, this number fluctuates between $1$ and $d$, influenced by the values of the counters at that particular step. Consequently, after $T$ rounds, the average counter value in \texttt{Pod} is precisely $T/m$, but in $\CMSCU$, it ranges between $T/m$ and $Td/m$. This variability in $\CMSCU$ makes computing the average counter value challenging, especially with the expansive state space of the underlying Markov process, let alone computing the approximate counting error.




\subsection{Contributions}



\emph{First}, we establish that, without any statistical assumptions on the stream, items absent from the stream exhibit the highest expected error within $\CMSCU$. This result reinforces empirical observations from previous studies~\cite{bianchi2012modelingCMSCU,MAZZIANE2022CMSCU} which highlights that infrequent items experience greater errors compared to other items.





\emph{Second}, we provide a new interpretation to the uniform counters selection assumption in $\CMSCU$. We note that under ideal hash functions, this assumption is akin to considering a specific stream where each item appears at most once. This interpretation sheds insights into the observed phenomenon that the expected error, of items absent from the stream, is maximal when counters are selected uniformly. We conjecture that this statement holds and defer its formal proof for future work.





\emph{Third}, we establish novel lower and upper bounds, parametrized by a positive integer~$g$, on the approximation error of $\CMSCU$ under uniform counter selection. These bounds correspond to the errors in two variants of $\CMS$ (\texttt{CU-LB} in Alg.~\ref{alg:LB-CBF-CU} and \texttt{CU-UB} in Alg.~\ref{alg:UB-CBF-CU}), where the \emph{counters gap}, i.e., the difference between the values of the maximal and minimal counter, is at most~$g$. This limited gap property permits the computation of the error by studying the dynamics of Markov chains with a state space of size $\binom{m+g-d}{m}$ and a sparse transition probabilities matrix. Specifically, the number of non-zero entries in the matrix is $\mathcal{O}\left(m\binom{m+g-d}{m}\right)$. 









% TODO: Outline of the proof
% 1. The error of CMS-CU is bounded by the errors of \texttt{CU-UB} and \texttt{CU-LB}
% 2. 



The reminder of this paper is organized as follows. 



==> Introductions/introduction_March.tex <==
Consider a dynamically changing vector~$\mathbf{n}= (n_i)_{i\in \mathcal{I}}$, where~$\mathcal{I}$ is a countable set. This vector~$\mathbf{n}$ undergoes updates based on a stream of pairs in $\mathcal{I}\times \mathbb{R}$, denoted as $((r_{t},v_t))_{t\in \mathbb{N}}$. At each time step $t$, the value~$n_{r_t}$ is incremented by~$v_t$. The objective is to quickly answer queries regarding functions of~$\mathbf{n}$ at any time~$t$, without storing $\mathbf{n}$, due to its large dimensionality. These queries may include estimating~$n_i$, the number of non-null entries in~$\mathbf{n}$, and calculating the~$L_p$ norm of~$\mathbf{n}$. Popular classic algorithms for approximately answering such queries include \textit{HyperLogLog}~\cite{flajolet2007hyperloglog}, \textit{Count-Sketch}~\cite{CHARIKAR2004CountSketch}, and \textit{Count-Min} (CM)~\cite{cormode2005improved}.



% Many of the proposed algorithms for  build on the classical \textit{Count-Min Sketch} (CM). 


In the particular case, where~$\mathbf{n}$ is initially equal to~$\mathbf{0}$, and~$v_t$ is always equal to~$1$, $\mathbf{n}$ counts the number of appearances of each item in the stream. CM is widely used in this context for network measurement~\cite{Basat2021Salsa}, anomaly detection~\cite{AnomalyDetectionCMS2021}, and the identification of frequently requested items in caching policies~\cite{TinyLFU2017}. Furthermore, CM is a building block for recently proposed algorithms for approximating~$\mathbf{n}$~\cite{DiamondSketch2019,HeavyKeeper2019}.





% M is widely used across various domains. A typical application of CM is approximately counting the number of appearances of a given item in massive data stream 


% applications being the efficient counting of the number of times a given item appears in a massive data stream~\cite{DiamondSketch2019}. This counting operation is crucial in tasks such as network measurement~\cite{Basat2021Salsa}, anomaly detection~\cite{AnomalyDetectionCMS2021}, and the identification of frequently requested items in caching policies~\cite{TinyLFU2017}. 




% maintains a compact representation of $\mathbf{n}$, offering a tread













  

 


% At each time step~$t$, the component corresponding to an item~$r_t\in \mathcal{I}$ is incremented by a value~$v$, i.e.,~$n_{r_t}(t) = n_{r_t}(t-1) + v$.



CM~\cite{cormode2005improved} stores a counters matrix with~$w$ columns and~$d$ rows and employs~$d$ hash functions~$h_1 , \ldots h_d$, drawn uniformly at random from a predefined family. Each hash function~$h_l$ maps each item to a single counter in row~$l$, namely~$(l,h_l(i))$. Initially, all counters are equal to~$0$ to represent the vector~$\mathbf{0}$. For each update~$(r_t,1)$ to~$\mathbf{n}$, CM increments all~$d$ counters associated to~$n$, namely~$(1,h_{1}(r_t), \ldots , (d,h_d(r_t))$, by~$1$. The estimation~$\hat n_i$ of~$n_i$ is the minimum value across item~$i$'s counters. In practice, the dimension of~$\mathbf{n}$ is larger than~$w$, resulting in multiple items hashing to the same counter and leading to an overestimation of~$n_i$. The tradeoff between the memory cost and the accuracy of CM is well understood under different assumptions on the stream~\cite{cormode2005improved,CormodeZipfErrorCMS2005}. In particular, for any stream, the estimation error for an item~$i$ at time~$t$, namely~$e_{i}(t)= \hat {n}_{i}(t) - n_{i}(t)$, is at most~$at/w$ with probability at least~$1-a^{-d}$ for any~$a>0$~\cite{cormode2005improved}.



A similar data structure to CM is the \textit{Spectral Bloom Filter} (SBF)~\cite{SpectralBloomFilters2003}. SBF stores a vector of~$M$ counters and employs~$d$ hash functions~$h_1,\ldots ,h_d$. Each hash function $h_l$ assigns to each item~$i$ a counter $h_l(i)$ in $\abIntInterval{1}{M}$. The counter updates in SBF follow the same process as in CM. Error analysis in both SBF and CM often relies on similar methodologies. Therefore, we treat SBF and CM interchangeably, referring to both as CM.



% The distinction lies in the fact that while in CM, hash function domains are disjoint, in the Spectral Bloom Filter all hash function domains is equal 
%  A similar data structure to CMS is the Spectral Bloom Filter, introduced in~\cite{SpectralBloomFilters2003}, with the only difference that the~$d$ hash functions domains are all equal to~$\abIntInterval{1}{M}$, denoted simply $\aIntInterval{M}$.







% Upon a query for $n_i$, CM estimates it with the minimum value across item~$i$'s counters.


% associated to the item~$r_t$ by $1$.



% to map each item to~$d$ counters, one from each row.  


% estimates~$n_i$ with the minimum value across item~$i$'s counters. 


% To answer a query for $\mathbf{n}_{i}$, 



% is an online algorithm that maintains a compact representation of the high dimensional vector~$\mathbf{n}$. CM stores $M=w\cdot d$ counters and maps each item to~$d$ counters via hash functions.  



% For counting purposes,~$n_i(t)$ is the number of times the item~$i$ has been requested thus far, i.e.,~$n_{i}(t)=\sum_{s=1}^{t} \mathds{1}(r_s = i)$, where~$\mathds{1}(B)$ stands for the indicator function that the event~$B$ is true. To approximate $n_i(t)$, CMS maintains a vector $\mathbf{Y}=(Y_{j})_{j\in \abIntInterval{1}{M}}$ of $M$ counters and employs $d$ hash functions $h_1,\ldots, h_d$ such that each $h_l: \mathcal{I} \mapsto \abIntInterval{1+ (l-1)w}{lw}$, where $M=w\cdot d$. The hash functions are chosen uniformly from a predefined family such that for every item $i$, $h_l(i)$ can be considered a uniform random variable over its domain. Note that once the hash functions are selected, they do not change when processing the stream. Upon a request~$r_t$, CMS increments all counters in the set~$\{ h_l(r_t): l\in \aIntInterval{d}\}$ by~$1$. The estimate of the request count for an item~$i$, denoted~$\hat n_{i}(t)$, is the minimum value across counters in~$\{ h_l(r_t): l\in \aIntInterval{d}\}$. It is clear that $\hat n_{i}(t)$ overestimates~$n_{i}(t)$. 

 
 


An update rule, known as the \textit{Conservative Update}~\cite{ConservativeUpdate2002}, improves the accuracy of CM by avoiding unnecessary increments. The Conservative Update rule increments only counters attaining the minimum value among the selected ones, maintaining upper bounds on the count estimation. Let~$Y_{j}(t)$ be the value of counter~$j$ at time step $t$. Initially, all counters are equal to~$0$. At any time step~$t>0$, the counters update in CM with conservative updates (CU) is as follows, 
\begin{align}\label{e:DynamicsCU}
        \CBFCUElement{j}{t+1} =
        \begin{cases} 
                    \CBFCUElement{j}{t} + 1, &\text{if } j \in \argmin_{i\in S_t}
                    \CBFCUElement{i}{t}, \\
                    \CBFCUElement{j}{t}, & \text{otherwise.}
        \end{cases}
    \end{align}
where~$S_t$ is the set of selected counters at time~$t$, namely,~$S_t=  \left\{ h_l(r_t) : \; l\in \abIntInterval{1}{d}  \right\}$. Similarly to CM, the estimation~$\hat n_{i}$ of~$n_i$ is the minimum overall item~$i$'s counters. The dynamics of CU are more difficult to analyze than those of CM because a counter's updates depend on the state of other counters. Four papers~\cite{bianchi2012modelingCMSCU,GILBloomCMSCU,MAZZIANE2022CMSCU,fusy2023phase} ventured to study the advantages of the conservative update in CM. 




Bianchi et al.~\cite{bianchi2012modelingCMSCU} experimentally observed that frequent items have negligible errors, while non-frequent items share a common error. Simulations indicate that this common error is maximal when at each time step,~$d$ counters are selected uniformly at random. 
% $(S_t)_{t\in \mathbb{N}}$ are i.i.d. uniform random variables in the set~$\aIntInterval{M}^{d}= \{S\subset [M]: |S| = d \}$
Consequently, they proposed a method to approximate CU's dynamics under the assumption of uniform counter-selection
% ~$(S_t)_{t\in \mathbb{N}}$ being uniform random variables,
in the regime where~$d/M$ tends to~$0$. However, their method requires recursively solving a system of ordinary differential equations.









Einziger and Friedman~\cite{GILBloomCMSCU} studied CU when~$(r_t)_{t\in \mathbb{N}}$ are i.i.d. categorical random variables over the set of items~$\mathcal{I}$. In particular, they approximate CU's dynamics with a stack of Bloom Filters~\cite{BroderBloomFilter2003}. Unfortunately, their approach lacks formal proof and may fail to capture the conservative update advantages~\cite{MAZZIANE2022CMSCU}. 




Ben Mazziane et al.~\cite{MAZZIANE2022CMSCU} studied also CU, under the assumption that~$(r_t)_{t\in \mathbb{N}}$ are i.i.d. categorical random variables. Their analysis theoretically supports that frequent items barely suffer any error in comparison to nonfrequent ones.
However, their study overlooked the benefits of conservative updates for non-frequent items and situations where item request probabilities are similar.



Recently, Fusy and Kucherov~\cite{fusy2023phase} modeled the relation between items in~$\mathcal{I}$ and the counters of CU as an undirected~$d$-uniform hypergraph, where counters serve as vertices, and~$(h_l(i))_{l\in \aIntInterval{d}}$, for~$i\in \mathcal{I}$, represent edges. Their model assumes that this hash hypergraph is uniformly random within the set of $d$-uniform hypergraphs with $M$ vertices and $N=|\mathcal{I}|$ edges, following the Erdős–Rényi model. Under this assumption, they distinguish two error regimes in CU related to the peelability property of the hash hypergraph, when the requests~$(r_t)_{t\in \mathbb{N}}$ are i.i.d. uniform random variables over~$\mathcal{I}$. Specifically, they show that the relative error, namely $(\hat n_{i}(T)- n_{i}(T))/n_{i}(T)$, tends to zero with high probability (w.h.p.) as both~$T$ and~$N$ approach infinity, provided that~$N<\lambda_d M$, where~$\lambda_d$ denotes the peelability threshold of the hash hypergraph. Conversely, when $d=2$, it was shown that if~$N> \lambda_d M$, the relative error is lower bounded by a constant dependent on~$\lambda$ w.h.p. in~$M$ and~$T$.



In this paper, we analyze CU when the selected counters~$(S_t)_{t\in \mathbb{N}}$ are i.i.d. uniform random variables in the set~$\{S\subset \mathcal{I}: \; |S|=d \}$. Our contributions are twofold. First, we prove the error in CM is maximal under this selection method. Moreover, we provide empirical evidence that CU's error is also maximal in the same setup. Second, we prove new lower and upper bounds on the error in CU under the uniform counters selection. More specifically, 

\begin{theorem}
    Under the assumption that~$(S_t)_{t\in \mathbb{N}}$ are i.i.d. uniform random variables in the set~$\{S\subset \abIntInterval{1}{M}: \; |S|=d \}$, for any $g\in \mathbb{N}$, the error for an item~$i$ with $n_{i}(T)=0$ in CU, satisfies,
    \begin{align}
 l_{g}(T)   \leq   \E{e_{i}(T)/T} \leq U_{g}(T),
\end{align}
where~$(l_{g}(T))_g$ and~$(U_{g}(T))_g$ are increasing and decreasing sequences in~$g$, respectively. Moreover, $l_g(T)=U_g(T)$ for any~$g\geq T$, leading to an exact expression of the expected error. The sequences~$l_{g}(T)$ and~$U_{g}(T)$ can be computed, recursively in~$T$, with time complexity~$\mathcal{O}(T M^{g+2})$. 
\end{theorem}
Numerical simulations show that the difference between~$U_g(T)$ and~$l_g(T)$ remains marginal, even for values of~$g$ much smaller than~$M$. For large values of~$T$ and for any~$g\in \mathbb{N}$, we show that~$e_{i}(T)/T$ concentrates around the interval~$[l_{g}(\infty), U_{g}(\infty)]$, where $l_{g}(\infty)$ and~$ U_{g}(\infty)$ corresponds to the limits of $l_{g}(T)$ and $U_g(T)$ when $T$ tends to infinity. Formally, 



\begin{theorem}
Under the assumption that~$(S_t)_{t\in \mathbb{N}}$ are i.i.d. uniform random variables in the set~$\{S\subset \abIntInterval{1}{M}: \; |S|=d \}$, for any $g\in\mathbb{N}$, the error for an item~$i$ with $n_{i}(T)=0$ in CU, satisfies,
    \begin{align}
\lim_{T \to +\infty} \Proba{l_{g}(\infty)   \leq   e_{i}(T)/T \leq U_{g}(\infty)} = 1.
\end{align}

\end{theorem}


% accurately estimates the expected error for values of~$g$ much smaller than~$M$. 




% Similarly to prior work~\cite{bianchi2012modelingCMSCU}, we provide experimental results supporting that the error in CU is maximal when counters are selected uniformly at random at each step. Moreover, we prove that the error is maximal in CM under the uniform counters selection. 


%  Furthermore, we prove that $e_{i}(T)/T$ is between the limits of $l_{g}(T)$ and $U_{g}(T)$ when $T\to +\infty$ with high probability in $T$. Formally, 

% Finally, we provide experiments supporting that the error is maximal in CMS-CU in the uniform counters selection setting. 










% Another result is proving the existence of $U_{g}(\infty)$ and $l_{g}(\infty)$ and the high probability bounds in $T$. 


% The computation of these limits requires computing the limiting distributions of ergodic Markov chains of state space $\mathcal{O}(M^{g+1})$ and with diameter~$M$

  % We stress that our results are better than the ones in~\cite{bianchi2012modelingCMSCU} as we provide formal proof of the upper bounds and lower bounds. 


==> Problems/preliminaries.tex <==
We consider a CU to approximate the number of appearances of items from a countable set~$\mathcal{I}$ in a stream $\mathbf{r}=(r_t)_{t\in \aIntInterval{T}}\in \mathcal{I}^{T}$, where~$\aIntInterval{n}$ designates the set~$\{1,\ldots, n \}$ for any positive integer~$n$. The number of appearances of an item~$i$ in the stream at time~$t$, denoted as~$n_{i}(t)$, is formally defined as~$n_{i}(t) = \sum_{s=1}^{t} \mathds{1}(r_s=i)$, where~$\mathds{1}(B)$ stands for the indicator function that the event~$B$ is true.

Let~$M$ be the total number of counters in CU, and~$h_{l}:\mathcal{I}\mapsto \aIntInterval{M},~l\in\aIntInterval{d}$, are hash functions drawn uniformly at random from a predefined family. Note that once the hash functions are selected, they do not change when processing the stream. We denote the value of CU's counters at time step~$t$ as~$\CBFCU{t}= \left( \CBFCUElement{j}{t}\right)_{j\in \aIntInterval{M}}$. Equation~\eqref{e:DynamicsCU} describes the dynamics of CU. Let~$\hat n_{i}(t)$ be the estimation of~$n_i(t)$ in CU, it follows that,~$\hat n_{i}(t) = \min_{l\in \aIntInterval{d}} \CBFCUElement{h_{l}(i)}{t}$.

The randomness in CU and CM stems from the choice of the hash functions. The performance analysis of hash-based data structures depends on the family from which hash functions are sampled. Often, it is desirable for $h_l(x)$ to be a uniform random variable over the domain $\aIntInterval{M}$ for any item $x$. Ideally, $(h_l(i))_{i\in \mathcal{I}}$ are mutually independent random variables, however, hash functions with such properties are time and memory-expensive. In practice, hash-based data structures operate with the lightweight 2-universal hash functions, i.e., $\Proba{h_l(x) = h_l(y)}\leq 1/M$ for any two distinct items~$x$ and~$y$. Nonetheless, Mitzenmacher and Vadhan~\cite{mitzenmacher2008simple} explain why the idealized hash functions model may predict the performance of 2-universal hash functions algorithms. 

In this work, we focus on CU's dynamics under the following assumption. 
    \begin{assumption}\label{assum:UniformCounters}
        The sets $(S_t)_{t\in \mathbb{N}}$, where $S_t=\{ h_l(r_t): l\in \aIntInterval{d} \}$, are i.i.d. uniform random variables over the set $\binom{\aIntInterval{M}}{d}= \{S\subset \aIntInterval{M}: \; |S|=d \}$. 
    \end{assumption}
Bianchi et al.~\cite{bianchi2012modelingCMSCU} studied CU's dynamics under the same assumption, as it aligns with experimental observations indicating a worst-case error scenario. More specifically, their simulations suggest that the expected error of an item~$i$ at time~$t$ in CU tends to increase as~$n_{i}(t)$ decreases. Notably, nonfrequent items are estimated with the same value, called \textit{error floor}. Moreover, it was observed that the error floor is maximal under Assumption~\ref{assum:UniformCounters}. 

One direct approach to study CU under Assumption~\ref{assum:UniformCounters} is to recognize that~$(\mathbf{Y}(t))$ forms a discrete-time Markov chain, allowing for the computation of the probability that~$\mathbf{Y}(t)$ is in a specific state. However, the state space of this Markov chain grows fast with~$t$. Bianchi et al.~\cite{bianchi2012modelingCMSCU} opted for an alternate representation to~$(\mathbf{Y}(t))$, taking advantage of counters being statistically indistinguishable. More specifically, they consider the process~$\boldsymbol{\psi}(\tau)= (\psi_l(\tau))_{l\in \mathbb{N}}$, where~$\psi_l(\tau) = \sum_{j=1}^{M} \mathds{1}\left( \CBFCUElement{j}{\tau M/d} \geq l \right)/ M$, and~$\tau$ takes values in~$\{kd/M:\; k\in \mathbb{N}  \}$. In the regime where~$d/M$ tends to~$0$, they capture the dynamics of~$\boldsymbol{\psi}(\tau)$ by a continuous deterministic function, which is the solution to a system of ordinary differential equations. 

This work formally proves that for any stream, the maximal expected error at time~$t$ in CU occurs for items with the lowest count, i.e., any item~$i_0$ such that~$n_{i_0}(t)=0$. Moreover, we prove that selecting~$d$ counters uniformly at random at each time step within CM maximizes the expected error for items such that~$n_{i_0}(t)=0$. We conjecture that a similar result holds for CU. Finally, we derive computationally efficient lower and upper bounds on the error valid for any values of~$d$ and~$M$. 


==> Problems/problem_15April.tex <==
Consider a dynamically changing vector~$\bm{n}(t)= (n_i(t))_{i\in \mathcal{I}}$, where~$\mathcal{I}$ is a countable set. This vector~$\mathbf{n}$ undergoes updates based on a stream of items in $\mathcal{I}$, denoted as $(r_{t})_{t\in \mathbb{N}}$. At each time step $t$, the value~$n_{r_t}$ is incremented by~$1$. The vector $\bm{n}(t)$ is formally defined as~$n_{i}(t) = \sum_{s=1}^{t} \mathds{1}(r_s=i)$, where~$\mathds{1}(B)$ stands for the indicator function that the event~$B$ is true.

The objective is to quickly answer queries regarding functions of~$\bm{n}$ at any time~$t$, without storing $\mathbf{n}$, due to its large dimensionality. These queries may include estimating~$n_i$, the number of non-null entries in~$\bm{n}$, and calculating the~$L_p$ norm of~$\bm{n}$. In this work we focus on estimating $\bm{n}(t)$, and we use $\hat{\bm{n}}(t)$ to denote its estimator at time $t\geq0$. We denote the error resulting from using $\hat{n}_{i}(t)$ for estimating ${n}_{i}(t)$ as $e_{i}(t)$. The estimation error $e_i(t)$ is then equal to $\hat n_{i}(t) - n_{i}(t)$.  

The Count-Min Sketch is a probabilistic data structure used for summarizing data streams and estimating the frequency of elements within them.
The sketch is initialized with parameters determining its size and resolution, and it's implemented as a 2-dimensional array, $\bm{Y} \in\mathbb{N}^{d\times m}$, where each row represents a hash function $h_{l}:\mathcal{I}\mapsto \aIntInterval{m},~l\in\aIntInterval{d}$, drawn uniformly at random from a predefined family of pairwise independent hash functions. Hash functions map items to specific column in the array, and as elements arrive, corresponding counters are updated. To estimate frequencies, the sketch performs lookups by hashing elements and retrieving the minimum value among the counters. Formally, $\hat{n}_{i}(t) \triangleq \min_{l \in[d]} Y_{d, h_{d}(l)}$.  Without loss of generality, we consider a one-dimensional Count-Min sketch,~i.e.,~$w=1$. It follows that,~$\hat n_{i}(t) = \min_{l\in \aIntInterval{d}} \CBFCUElement{h_{l}(i)}{t}$. 

The Conservative Update  rule increments only counters attaining the minimum value among the selected ones, maintaining upper bounds on the count estimation. At any time step~$t>0$, the counters update in \texttt{CMS-CU} is as follows, 
\begin{align}\label{e:DynamicsCU}
        \CBFCUElement{j}{t+1} =
        \begin{cases} 
                    \CBFCUElement{j}{t} + 1, &\text{if } j \in \argmin_{i\in S_t}
                    \CBFCUElement{i}{t}, \\
                    \CBFCUElement{j}{t}, & \text{otherwise.}
        \end{cases}
    \end{align}
where~$S_t$ is the set of selected counters at time~$t$, namely,~$S_t=  \left\{ h_l(r_t) : \; l\in \abIntInterval{1}{d}  \right\}$. 



==> Problems/problem_March.tex <==
Consider a dynamically changing vector~$\mathbf{n}= (n_i)_{i\in \mathcal{I}}$, where~$\mathcal{I}$ is a countable set. This vector~$\mathbf{n}$ undergoes updates based on a stream of pairs in $\mathcal{I}\times \mathbb{R}$, denoted as $((r_{t},v_t))_{t\in \mathbb{N}}$. At each time step $t$, the value~$n_{r_t}$ is incremented by~$v_t$. The objective is to quickly answer queries regarding functions of~$\mathbf{n}$ at any time~$t$, without storing $\mathbf{n}$, due to its large dimensionality. These queries may include estimating~$n_i$, the number of non-null entries in~$\mathbf{n}$, and calculating the~$L_p$ norm of~$\mathbf{n}$. 

CM~\cite{cormode2005improved} stores a counters matrix with~$w$ columns and~$d$ rows and employs~$d$ hash functions~$h_1 , \ldots h_d$, drawn uniformly at random from a predefined family. Each hash function~$h_l$ maps each item to a single counter in row~$l$, namely~$(l,h_l(i))$. Initially, all counters are equal to~$0$ to represent the vector~$\mathbf{0}$. For each update~$(r_t,1)$ to~$\mathbf{n}$, CM increments all~$d$ counters associated to~$n$, namely~$(1,h_{1}(r_t), \ldots , (d,h_d(r_t))$, by~$1$. The estimation~$\hat n_i$ of~$n_i$ is the minimum value across item~$i$'s counters. In practice, the dimension of~$\mathbf{n}$ is larger than~$w$, resulting in multiple items hashing to the same counter and leading to an overestimation of~$n_i$. The tradeoff between the memory cost and the accuracy of CM is well understood under different assumptions on the stream~\cite{cormode2005improved,CormodeZipfErrorCMS2005}. In particular, for any stream, the estimation error for an item~$i$ at time~$t$, namely~$e_{i}(t)= \hat {n}_{i}(t) - n_{i}(t)$, is at most~$at/w$ with probability at least~$1-a^{-d}$ for any~$a>0$~\cite{cormode2005improved}.

A similar data structure to CM is the \textit{Spectral Bloom Filter} (SBF)~\cite{SpectralBloomFilters2003}. SBF stores a vector of~$M$ counters and employs~$d$ hash functions~$h_1,\ldots ,h_d$. Each hash function $h_l$ assigns to each item~$i$ a counter $h_l(i)$ in $\abIntInterval{1}{M}$. The counter updates in SBF follow the same process as in CM. Error analysis in both SBF and CM often relies on similar methodologies. Therefore, we treat SBF and CM interchangeably, referring to both as CM.

An update rule, known as the \textit{Conservative Update}~\cite{ConservativeUpdate2002}, improves the accuracy of CM by avoiding unnecessary increments. The Conservative Update rule increments only counters attaining the minimum value among the selected ones, maintaining upper bounds on the count estimation. Let~$Y_{j}(t)$ be the value of counter~$j$ at time step $t$. Initially, all counters are equal to~$0$. At any time step~$t>0$, the counters update in CM with conservative updates (CU) is as follows, 
\begin{align}\label{e:DynamicsCU}
        \CBFCUElement{j}{t+1} =
        \begin{cases} 
                    \CBFCUElement{j}{t} + 1, &\text{if } j \in \argmin_{i\in S_t}
                    \CBFCUElement{i}{t}, \\
                    \CBFCUElement{j}{t}, & \text{otherwise.}
        \end{cases}
    \end{align}
where~$S_t$ is the set of selected counters at time~$t$, namely,~$S_t=  \left\{ h_l(r_t) : \; l\in \abIntInterval{1}{d}  \right\}$. Similarly to CM, the estimation~$\hat n_{i}$ of~$n_i$ is the minimum overall item~$i$'s counters. The dynamics of CU are more difficult to analyze than those of CM because a counter's updates depend on the state of other counters. Four papers~\cite{bianchi2012modelingCMSCU,GILBloomCMSCU,MAZZIANE2022CMSCU,fusy2023phase} ventured to study the advantages of the conservative update in CM. 



==> assumption.tex <==
There are two major sources of randomness within Count-Min Sketch and its hash-based variants. Firstly, randomness is introduced through the selection and distribution of hash functions. 
Ideally, these hash function, $(h_l(i))_{i\in \mathcal{I}}$, are chosen to be independent and uniformly distributed, in order to ensure  that elements in the stream are mapped to different positions within the sketch, miinimizing collisions and facilitating accurate frequency estimations. This property is formalized in Assumption~\ref{assum:IdealHash}.
\begin{assumption}{(Ideal Hash Functions Model)}\label{assum:IdealHash}
        The sets~$\left(\{h_l(i): l\in \llbracket d \rrbracket \} \right)_{i\in \mathcal{I}}$ are i.i.d. uniform random variables in the set~$\binom{\aIntInterval{m}}{d}$.
\end{assumption}
Assumption~\ref{assum:IdealHash} is a variation of the ideal hash functions model, ensuring that each item has exactly~$d$ counters for any random selection of hash functions.
Hash functions with such properties are time and memory-expensive. In practice, hash-based data structures operate with the lightweight 2-universal hash functions, i.e., $\Proba{h_l(i) = h_l(j)}\leq 1/m$ for any two distinct items~$i,j\in\mathcal{I}$.  Nonetheless,~\cite{mitzenmacher2008simple} explains why the idealized hash functions model may predict the performance of 2-universal hash functions algorithms. 

Secondly, the inherent randomness in the data stream itself adds another layer of stochasticity to the process. Ideally, when the catalog of item is infinite w.r.t the time horizon, i.e., $T \ll |\mathcal{I}|$, it is unlikely that the same item would be requested more than once. Assumption~\ref{assum:DistinctRequests} formalizes this ideal distinct request property. 
\begin{assumption}\label{assum:DistinctRequests}
    The stream~$\mathbf{r}$ consists of distinct items, i.e.,~$r_t\neq r_s$ for every~$t\neq s\in \aIntInterval{T}$.
\end{assumption}
Interestingly, thanks to Assumption~\ref{assum:IdealHash}, for any two items~$i, j\in\mathcal{I}$ not appearing in the stream before time~$t>0$, the errors~$e_{i}(t)$ and~$e_{j}(t)$ are identically distributed. Let~$e^{*}(t)$ denote a random variable following their common probability distribution. While Assumption~\ref{assum:DistinctRequests} does not usually hold, it serves in upper-bounding the estimation error, as shown in Proposition~\ref{prop:WorstErrorItemNotReq}.
\begin{proposition}\label{prop:WorstErrorItemNotReq}
    Under Assumption~\ref{assum:IdealHash}, the error for any item~$i\in \mathcal{I}$ in CU satisfies, 
        \begin{flalign}
             \E{e_{i}(T)} \leq \E{e^{*}(T)}, \; \forall T. 
        \end{flalign}
    where the expectation is taken over the random choice of the hash functions. 
\end{proposition}
Proposition~\ref{prop:WorstErrorItemNotReq} formally proves that for any stream, the maximal expected estimation error at time~$t$ occurs for items with the lowest count, i.e., any item~$i_0$ such that~$n_{i_0}(t)=0$. 

Experimental findings in~\cite{bianchi2012modelingCMSCU,MAZZIANE2022CMSCU} suggest that the expected error of an item~$i$ at time~$t$ in \texttt{CMS-CU} tends to increase as~$n_{i}(t)$ decreases. This observation finds partial validation in Proposition~\ref{prop:WorstErrorItemNotReq}; it shows that, across all possible streams, the error is maximal for any item~$i_{0}$ that was not requested before time~$t$, i.e.,  when~$n_{i_0}(t)=0$. Notably, in~\cite{bianchi2012modelingCMSCU}, non-frequent items are estimated with the same value, called \emph{error floor}. In the context of our Proposition~\label{prop:WorstErrorItemNotReq}, $e^{*}(T)$ is the error floor.


Additionally, the experiments in~\cite{bianchi2012modelingCMSCU} indicate that~$\E{e^{*}(t)}$ reaches its maximum when~$d$ distinct counters are uniformly selected at random during each time step. This uniform counters property is formalized in Assumption~\ref{assum:UniformCounters}. 
\begin{assumption}\label{assum:UniformCounters}
    The sets $(S_t)_{t\in \mathbb{N}}$, where $S_t=\{ h_l(r_t): l\in \aIntInterval{d} \}$, are i.i.d. uniform random variables over the set $\binom{\aIntInterval{m}}{d}= \{S\subset \aIntInterval{m}: \; |S|=d \}$. 
\end{assumption}

Assumption~\ref{assum:UniformCounters} can be interpreted as a consequence of Assumptions~\ref{assum:IdealHash} and~\ref{assum:DistinctRequests}. In the sense\dots. In the reminder of the paper, we focus on scenarios where Assumption~\ref{assum:UniformCounters} holds.

% We conjecture that 


\paragraph*{Added paragraph}

$\CMSCU$ is a randomized algorithm due to the choice of the hash functions uniformly at random from a specific family. In general,  the performance analysis of hash-based data structures, e.g., the estimation error for $\CMSCU$, depends on the family from which hash functions are sampled. Ideally, $(h_l(i))_{i\in \mathcal{I}}$ are mutually independent random variables, however, hash functions with such properties are time and memory-expensive. In practice, hash-based data structures operate with the lightweight 2-universal hash functions, i.e., $\Proba{h_l(i) = h_l(j)}\leq 1/m$ for any two distinct items~$i,j\in \mathcal{I}$. Nonetheless, Mitzenmacher and Vadhan~\cite{mitzenmacher2008simple} explain why the idealized hash functions model often predicts in practice the performance of 2-universal hash functions algorithms. This paper considers a variant of the idealized hash functions model, ensuring that each item is mapped to exactly~$d$ counters. This property is formalized in Assumption~\ref{assum:IdealHash}.

==> draft.tex <==
\section{draft main results}


\subsubsection{Lower bound process}

The lower bound process yields, 

    \begin{align}
            \pi_{0}^{\text{lb},g} = \frac{(m-2)(m-1)^{g}}{2(m-1)^{g+1} - m}, 
            \; \pi_{f}^{\text{lb},g} =\frac{m(m-2)(m-1)^{g-f}}{2(m-1)^{g+1} - m},\; \forall f \in \aIntInterval{g}.
    \end{align}



\subsection{The case where g is equal to 1.} 
First define the constants $\alpha_k$ and $\beta_k$ as follows, 

    \begin{align}
            \alpha_k = \frac{\binom{m-k}{2}}{\binom{m}{2}}, \; \beta_k = \frac{\binom{k}{1}\binom{m-k}{1}}{\binom{m}{2}}
    \end{align}
The limiting distribution satisfies,
    \begin{align}
            &\pi_k = \alpha_{m-k} \pi_k + \alpha_{k-2} \pi_{k-2} + \beta_{k-1} \pi_{k-1}, \forall k\in \{2,\ldots , M-1 \}, \\
            &\pi_2 = \alpha_{m-2} \pi_2 + \alpha_{0} \pi_0 \\  
            &\pi_0 = \alpha_{m-2} \pi_{m-2} + \beta_{m-1} \pi_{m-1} \\ 
            &\sum_{i} \pi_i = 1. 
    \end{align}

\subsection{Columns}

\paragraph*{Columns of the transition matrix.}The number of non-zero entries in the column corresponding to the vector~$\mathbf{k}$ coincides with the number of solutions to the equation~$\LBGamma(\mathbf{q}, v,c )= \mathbf{k}$, where $(\mathbf{q}, v,c)\in \Omega_g \times \abIntInterval{0}{g} \times \aIntInterval{d}$. We distinguish three cases. 

\begin{enumerate}
    \item If~$v\notin \{0, g\}$, then for each~$c\leq k_{v+1}$, there exists a unique vector~$\mathbf{q}\in \Omega_g$ such that~$\LBGamma(\mathbf{q}, v,c )= \mathbf{k}$ (see~\eqref{e:LBSTransCU}). Indeed, $q_{v}=k_v + c$, $q_{v+1}=k_{v+1}-C$ and $q_l=k_l$ for any $l\notin {v,v+1}$. Consequently, the count of solutions in this case is less than~$m$.

    \item When~$v=g$, the unique solution is~$(\mathbf{k}, g,d)$. 

    \item For the case where $v = 0$, $\LBGamma(\mathbf{q}, 0, c)$ has two possible expressions (see~\eqref{e:LBTransCUVZero} and~\eqref{e:LBSTransCU}), resulting in at most two potential solutions for each value of~$c$. The first solution, derived from~\eqref{e:LBSTransCU}, occurs when $c \leq k_1$ and is characterized by $q_0 = k_0 + c$, $q_1 = k_1 - c$, and $q_l = k_l$ for any other $l$. The second solution, stemming from~\eqref{e:LBTransCUVZero}, arises when~$c \leq k_0$, and is described by~$q_0 = c$, $q_1 = k_0 - c$, and~$q_l = k_{l-1}$ for other~$l$. Consequently, the number of solutions in this scenario is at most~$2d$. 
\end{enumerate}
We deduce that the number of columns is limited to~$\mathcal{O}(m)$. 


The number of non-zero entries in the column corresponding to the vector~$\mathbf{k}$ in the matrix $\UBMatrixTrans{g}$ coincides with the number of solutions to the equation~$\UBGamma(\mathbf{q}, v,c )= \mathbf{k}$, where $(\mathbf{q}, v,c)\in \Omega_g \times \abIntInterval{0}{g} \times \aIntInterval{d}$. We distinguish two cases. 

% \begin{enumerate}
%     \item If~$v\neq g$, then $\UBGamma(\mathbf{k},v,c) = \LBGamma(\mathbf{k},v,c)$ and therefore the number of solutions is $\mathcal{O}(m)$. 

%     \item When~$v=g$, $c$ is equal to~$d$, and solutions exist only if~$k_g=d$.  In this case, $q_g=k_{g-1}+d$, $q_l=k_{l-1}$, $\forall l \in \abIntInterval{2}{g-1}$, and $q_0+q_1=k_0$. It follows that the number of solutions is at most~$m$. 
% \end{enumerate}
% We deduce that the number of columns is limited to~$\mathcal{O}(m)$.




















\begin{proposition}
Let~$\mathbf{r}^{*}$ be a stream that satisfies Assumption~\ref{assum:DistinctRequests}. Under Assumption~\ref{assum:IdealHash}, the expected value of~$e^{*}_{\text{CM}}(t, \mathbf{r})$ is maximal for $\mathbf{r}=\mathbf{r}^{*}$. Formally, 


any stream $\mathbf{r}^{*}$ that satisfies Assumption~\ref{assum:DistinctRequests}, maximizes the expected value of~$e^{*}_{\text{CM}}(t, \mathbf{r})$. Formally, 
\begin{align}
        \mathbf{r}^{*} \in \argmax_{\mathbf{r} \in \mathcal{I}^{\mathbb{N}}} \E{e^{*}_{\text{CM}}(t, \mathbf{r})}.
\end{align}
% Moreover,~$\E{e^{*}_{\text{CM}}(t, \mathbf{r})}$ is equal to the expected value of any counter in CU, under Assumption~\ref{assum:UniformCounters}. 
\end{proposition}
\begin{proof}

We fix an item~$j$ with~$n_{j}(t)=0$. We define~$U= \{r_s : \; s\in \aIntInterval{t}\}$. Observe that for any two hash functions~$\mathbf{h}$ and~$\mathbf{g}$, such that~$g_l(i)=h_l(i)$ for any~$l$ and~$i\in U$, counters in CM at time~$t$ are equal, i.e.,~$\mathbf{Y}(\mathbf{h}, t)=\mathbf{Y}(\mathbf{g}, t)$. Let~$\mathbf{o}$ be a hash function mapping~$U$ to~$\binom{\aIntInterval{M}}{d}$. 
We define the set $\mathcal{N}(\mathbf{o})$ as follows, 
    \begin{align}
            \mathcal{N}(\mathbf{o}) = \left\{ \mathbf{h}\in \mathcal{H}: \; h_l(i)=o_l(i), \; \forall i,l \in U\cup\{j\} \times \aIntInterval{d} \right\}.  
    \end{align}

Let~$\sigma_{\mathbf{o}}$ be permutation for~$\aIntInterval{M}$ that sorts the counters when the chosen hash function~$\mathbf{h}$, satisfies $h_l(i)=o_l(i)$, for any~$l$ and~$i\in U$. Specifically, $\mathbf{Y}(\mathbf{h},\sigma_{\mathbf{o}}(r)) \leq \mathbf{Y}(\mathbf{h},\sigma_{\mathbf{o}}(r+1))$. 

\end{proof}



\paragraph{CMS.} We have that $\E{\CBFCUElement{i}{T}} \geq \E{\CBFCUElement{i+1}{T}}$. Moreover, in CMS, we have always, 
    \begin{align}
        \sum_{j=1}^{M} Y_{j}(T) = d\cdot T. 
    \end{align}
Therefore it is easy to see that the average error in CMS is maximized when $\E{\CBFCUElement{i}{T}} = \E{\CBFCUElement{j}{T}} = T\cdot \frac{d}{M}$ for any $i,j \in [M]$. This can only be verified if the sequence of requests has no repetition, i.e., $r_t \neq r_s, \; \forall s,t \in [T]$.  This case is equivalent to choosing $S_t$ uniformly at random from the set~$\left\{ S\in [M]:  \# S = d\right\}$. 

\paragraph{CMS-CU.} While we still have $\E{\CBFCUElement{i}{T}} \geq \E{\CBFCUElement{i+1}{T}}$, in CMS-CU we have only the inequality, 
    \begin{align}
        T  \leq     \sum_{j=1}^{M} Y_{j}(T) \leq d\cdot T. 
    \end{align}
Therefore the Growth is not constant 
    

The cardinality of the set $\Omega_g$ verifies the following bound~\cite{YavuzORUCPartitionInteger2016}, 

        \begin{align}
            \#  \left(  \Omega_g \right) \leq \frac{1}{2} \binom{M-1}{g} 
        \end{align}


==> estimation_errror/capped_sketch.tex <==
\begin{algorithm}[t]
\caption{\texttt{LB-CU}}
\begin{algorithmic}[1]
\State \textbf{Input:} $(S_t)_{t\in \aIntInterval{T}}$, $g$
\State  $\LBCBFCU{g}{0} \gets \mathbf{0}$
\For{$t$ in $\aIntInterval{T}$}
    \If{$\LBCBFCUElement{g}{\text{max}}{t-1}-\LBCBFCUElement{g}{\text{min}}{t-1} = g$, and $\min_{i\in S_t} \LBCBFCUElement{g}{i}{t-1}=\LBCBFCUElement{g}{\text{max}}{t-1}$}
        \State $\LBCBFCU{g}{t} \gets \LBCBFCU{g}{t-1}$ \label{line:LBNoUpdate}
    \Else
        \State $\LBCBFCU{g}{t} \gets$ \text{CU}$\left(\LBCBFCU{g}{t-1}, S_t\right)$ \label{line:LBCuUpdate}
    \EndIf
\EndFor
\end{algorithmic}
\label{alg:LB-CBF-CU}
\end{algorithm}

A key idea to prove Theorems~\ref{th:main} and~\ref{th:mainHPConcentration}, is to introduce two variants OF \texttt{CMS-CU}, which we call \texttt{LB-CU} and \texttt{UB-CU}. The dynamics of \texttt{LB-CU} and \texttt{UB-CU} are outlined in Algorithms~\ref{alg:LB-CBF-CU} and~\ref{alg:UB-CBF-CU}, respectively. Both variants feature a parameter~$g\in \mathbb{N}$. 
In \texttt{LB-CU}, we denote the counter values at step~$t$ as~$\LBCBFCU{g}{t}= (\LBCBFCUElement{g}{j}{t})_{j\in \aIntInterval{M}}$, and we denote the maximum and minimum counter values, namely~$\max_{j\in \aIntInterval{M}} \LBCBFCUElement{g}{j}{t}$ and~$\min_{j\in \aIntInterval{M}} \LBCBFCUElement{g}{j}{t}$, as~$\LBCBFCUElement{g}{\max}{t}$ and~$\LBCBFCUElement{g}{\min}{t}$, respectively.
We use a similar notation for \texttt{UB-CU}, by replacing the superscript ``$\text{lb}$'' with ``$\text{ub}$''.
Initially, all counters are equal to~$0$. At each step~$t\geq 1$,~$S_t=\{h_l(r_t):\; l\in \aIntInterval{d}\}$ represents the~$d$ selected counters. Both \texttt{LB-CU} and \texttt{UB-CU} update counter values based on the previous state, distinguishing between two cases:
  \begin{enumerate}
    \item If the gap between maximum and minimum counter values equals $g$, and all selected counters have values equal to the maximum counter value, \texttt{LB-CU} performs no updates (line~\ref{line:LBNoUpdate}), while in \texttt{UB-CU}, counters with values equal to $\UBCBFCUElement{g}{\text{min}}{t-1}$ are incremented (line~\ref{line:UbMinUpdate}), along with the selected counters (line~\ref{line:UbCuUpdate}).
    \item Otherwise, \texttt{LB-CU} and \texttt{UB-CU} update the counters according to the conservative update in~\eqref{e:DynamicsCU} (lines~\ref{line:LBCuUpdate} and~\ref{line:UbCuUpdate}). 
\end{enumerate}
Observe that for any stream of length~$T$ and any value $g\geq T$, \texttt{LB-CU}, \texttt{UB-CU}, and \texttt{CU} produce identical counter vectors, i.e., $\LBCBFCU{g}{t}=\UBCBFCU{g}{t}=\CBFCU{t}$, for any $t\in \aIntInterval{T}$. Similarly to~$e^{*}(t)$ in CU, we define~$\LBErrorstar{g}{t}$ and~$\UBErrorstar{g}{t}$ as errors with probability distributions identical to the error for any item~$i$ with~$n_{i}(t)=0$, in \texttt{LB-CU} and \texttt{UB-CU}, respectively.

\subsection{Expected Error of }
Efficient computation of both quantities relies on similar techniques. Therefore, we first introduce a method to compute~$\E{\LBErrorstar{g}{T}}/T$ and subsequently demonstrate how to adapt this method to calculate~$\E{\UBErrorstar{g}{T}}/T$. A key point of our method is to study the stochastic evolution of the number of counters that are far from the minimum value counter by any value~$l$, denoted~$\LBExcessEle{g}{l}(t)$. Formally,
\begin{align}\label{e:defExcessLBCU}
        \LBExcessEle{g}{l}(t) \triangleq \sum_{j=1}^{M} \mathds{1}\left( \LBCBFCUElement{g}{j}{t} - \LBCBFCUElement{g}{\min}{t} =l   \right).
\end{align}
Indeed, $(\LBExcess{g}(t)=( \LBExcessEle{g}{l}(t))_{l\in \mathbb{N}})_t$ is a time-homogeneous Markov chain with finite state space, denoted~$\Omega_g$. Moreover, the conditional expectation of~$\LBErrorstar{g}{t}-\LBErrorstar{g}{t-1}$ given~$(\LBExcess{g}(t), \LBExcess{g}(t-1)) = (\mathbf{k^{'}},\mathbf{k})$, is invariant with respect to~$t$, denoted as~$\LBProbaError{g}{k}{k^{'}}$.~Let $\LBMatrixError{g}$ be the matrix with components $\LBProbaError{g}{k}{k^{'}}$ for any $(\mathbf{k},\mathbf{k^{'}})\in (\Omega_g)^{2}$. $\LBMatrixTrans{g}$ denotes the one-step transition probabilities matrix of~$(\LBExcess{g}(t))_t$, $\LBOccupancyEle{g}{k}(t)$ represents the probability that $\LBExcess{g}(t)=\mathbf{k}$, and $\LBOccupancy{g}(t)$ is the vector of these probabilities for each state $\mathbf{k}\in \Omega_g$.

\begin{proposition}\label{prop:EfficientComputation}
The quantity~$\E{\LBErrorstar{g}{T}}$ satisfies, 
\begin{align}\label{e:ExpErrorLBg}
            \E{\LBErrorstar{g}{T}} = \left\langle  \sum_{t=0}^{T-1}\LBOccupancy{g}(t) ,  \LBMatrixTrans{g} \odot \LBMatrixError{g} \cdot \mathbf{1}^\intercal \right\rangle,
\end{align}
where~$\odot$ is the element-wise product, and~$\mathbf{1}^{\intercal}$ represents a column vector with $|\Omega_g|$ rows, where each entry is equal to~$1$. Furthermore, computing~$\E{\LBErrorstar{g}{T}}$ using~\eqref{e:ExpErrorLBg} incurs a time complexity of~$\mathcal{O}\left(\max(d,T) M \binom{M+g-d}{g}\right)$.
\end{proposition}   

\begin{proposition}\label{prop:HPConcentration}
    The random variable~$\LBErrorstar{g}{T}/T$ converges almost surely to constants as~$T$ tends to infinity. Formally, 

        \begin{align}
            \Proba{\lim_{T\to +\infty} \LBErrorstar{g}{T}/ T  = \left\langle  \LBOccupancy{g}(\infty) ,  \LBMatrixTrans{g} \odot \LBMatrixError{g} \cdot \mathbf{1}^\intercal \right\rangle} = 1, 
        \end{align}
where $\LBOccupancy{g}(\infty)$ is the limiting distribution of~$(\LBExcess{g}(t))_t$. 
\end{proposition}


\begin{algorithm}[t]
\caption{\texttt{UB-CU}}
\begin{algorithmic}[1]
\State \textbf{Input:} $(S_t)_{t\in \aIntInterval{T}}$, $g$
\State $\UBCBFCU{g}{0}  \gets \mathbf{0}$
\For{$t$ in $\aIntInterval{T}$}
    \State $\UBCBFCU{g}{t} \gets$ \text{CU}$\left(\UBCBFCU{g}{t-1}, S_t\right)$ \label{line:UbCuUpdate}
     \If{$\UBCBFCUElement{g}{\text{max}}{t-1}-\UBCBFCUElement{g}{\text{min}}{t-1} = g$, and $\min_{i\in S_t} \UBCBFCUElement{g}{i}{t-1}=\UBCBFCUElement{g}{\text{max}}{t-1}$}
        \State $\UBCBFCUElement{g}{j}{t}= \UBCBFCUElement{g}{j}{t-1} + 1, \; \forall j\in \aIntInterval{M}: \; \UBCBFCUElement{g}{j}{t-1}= \UBCBFCUElement{g}{\text{min}}{t-1}$\label{line:UbMinUpdate}
    \EndIf
\EndFor
\end{algorithmic}
\label{alg:UB-CBF-CU}
\end{algorithm}



==> estimation_errror/header.tex <==


 While Assumption~\ref{assum:DistinctRequests} does not usually hold, it serves in upper-bounding the estimation error, as shown in Proposition~\ref{prop:WorstErrorItemNotReq}.
\begin{proposition}\label{prop:WorstErrorItemNotReq}
    Under Assumption~\ref{assum:IdealHash}, the error for any item~$i\in \mathcal{I}$ in CU satisfies, 
        \begin{flalign}
             \E{e_{i}(T)} \leq \E{e^{*}(T)}, \; \forall T. 
        \end{flalign}
    where the expectation is taken over the random choice of the hash functions. 
\end{proposition}
Proposition~\ref{prop:WorstErrorItemNotReq}  formally proves that for any stream, the maximal expected estimation error at time~$t$ occurs for items with the lowest count, i.e., any item~$i_0$ such that~$n_{i_0}(t)=0$. 

Experimental findings in~\cite{bianchi2012modelingCMSCU,MAZZIANE2022CMSCU} suggest that the expected error of an item~$i$ at time~$t$ in \texttt{CMS-CU} tends to increase as~$n_{i}(t)$ decreases. This observation finds partial validation in Proposition~\ref{prop:WorstErrorItemNotReq}; it shows that, across all possible streams, the error is maximal for any item~$i_{0}$ that was not requested before time~$t$, i.e.,  when~$n_{i_0}(t)=0$. Notably, in~\cite{bianchi2012modelingCMSCU}, non-frequent items are estimated with the same value, called \emph{error floor}. In the context of our Proposition~\label{prop:WorstErrorItemNotReq}, $e^{*}(T)$ is the error floor.


Additionally, the experiments in~\cite{bianchi2012modelingCMSCU} indicate that~$\E{e^{*}(t)}$ reaches its maximum when~$d$ distinct counters are uniformly selected at random during each time step. This uniform counters property is formalized in Assumption~\ref{assum:UniformCounters}. 

One direct approach to study \texttt{CMS-CU} under Assumption~\ref{assum:UniformCounters} is to recognize that~$(\mathbf{Y}(t))$ forms a discrete-time Markov chain, allowing for the computation of the probability that~$\mathbf{Y}(t)$ is in a specific state. However, the state space of this Markov chain grows fast with~$t$. 
To deal with the growing state space, we introduce \texttt{CU-LB} (Algorithm~\ref{alg:LB-CBF-CU}) and \texttt{CU-UB} (Algorithm~\ref{alg:LB-CBF-CU}); two variants of \texttt{CMS-CU} where the \emph{counters gap}, i.e., the difference between the values of the maximal and minimal counter, is capped by a constant $g\in\mathbb{N}$.  

The approximation error of the constructed capped variants \texttt{CMS-CU} bounds the approximation error of  \texttt{CMS-CU} with a high probability, as shown in Theorem~\ref{th:mainHPConcentration}. In these two variants of \texttt{CMS-CU}, the counters gap is capped. Therefore, there dynamic can modeled as discrete-time Markov chain with finite state space. 

In the reminder of this section, we provide details on the construction of \texttt{CU-LB} and \texttt{CU-UB}, and we  

==> estimation_errror/main_result.tex <==
\begin{theorem}\label{th:main}
    Under Assumption~\ref{assum:UniformCounters}, for any~$g\in \mathbb{N}$, there exist positive values~$\ell_g(T)$ and~$U_g(T)$, such that the error~$e^{*}(T)$ satisfies,
\begin{align}
 \ell_{g}(T)   \leq   \E{e^{*}(T)/T} \leq U_{g}(T),
\end{align}
where~$(\ell_{g}(T))_g$ and~$(U_{g}(T))_g$ form strictly increasing and decreasing sequences for~$g<T$, respectively. Conversely, $\ell_g(T)=U_g(T)$ when~$g\geq T$. Furthermore, these quantities~$\ell_{g}(T)$ and~$U_{g}(T)$ can be computed with time complexity~$\mathcal{O}(\max(d,T) M\binom{M+g-d}{g})$. 

\end{theorem}

\begin{theorem}\label{th:mainHPConcentration}
Under Assumption~\ref{assum:UniformCounters}, for any~$g\in\mathbb{N}$, the error $e^{*}(T)$ satisfies, 
    \begin{align}
\lim_{T \to +\infty} \Proba{\ell_{g}(\infty)   \leq   e^{*}(T)/T \leq U_{g}(\infty)} = 1,
\end{align}
where~$\ell_{g}(\infty) = \lim_{T\to \infty} \ell_g(T)$ and~$U_{g}(\infty) = \lim_{T\to \infty} U_g(T)$. 
\end{theorem}

Theorem~\ref{th:mainHPConcentration} proves that~$e^{*}(T)/T$ concentrates around the interval~$[l_{g}(\infty), U_{g}(\infty)]$ for large values of~$T$. The values~$l_{g}(\infty)$ and~$U_{g}(\infty)$ can be approximated by the values of the sequences $l_{g}(T)$ and $U_{g}(T)$ for large values of~$T$. 


 


\begin{proposition}\label{prop:SandwichBound}
For any~$g\in \mathbb{N}$ and any sequence of selected counters~$(S_t)$, the error~$e^{*}(T)$ satisfies, 
    \begin{equation}\label{e:SandwichError}
       \LBErrorstar{g}{T}     \leq   e^{*}(T) \leq \UBErrorstar{g}{T}.
    \end{equation} 
Additionally, the sequences~$(\E{\LBErrorstar{g}{T}}/T)_g$ and~$(\E{\UBErrorstar{g}{t}}/T)_g$ are strictly increasing and decreasing sequences for~$g<T$, respectively. On the other hand, for any~$g\geq T$, both sequences converge to~$\E{e^{*}(T)/T}$. 
\end{proposition}   

Proposition~\ref{prop:SandwichBound} proves the first part of Theorem~\ref{th:main}, where~$\ell_g(T)$ and~$U_{g}(T)$ denote $\E{\LBErrorstar{g}{T}}/T$ and~$\E{\UBErrorstar{g}{T}}/T$ respectively. 

The proof of Theorem~\ref{th:main} readily follows from Propositions~\ref{prop:SandwichBound} and~\ref{prop:EfficientComputation}, while establishing Theorem~\ref{th:mainHPConcentration} is straightforward with Propositions~\ref{prop:SandwichBound} and~\ref{prop:HPConcentration}.


==> main_results/error_computation_1.tex <==

One direct approach to study \texttt{CMS-CU} under Assumption~\ref{assum:UniformCounters} is to recognize that~$(\mathbf{Y}(t))$ forms a discrete-time Markov chain, allowing for the computation of the probability that~$\mathbf{Y}(t)$ is in a specific state. However, the state space of this Markov chain grows fast with~$t$. 
To deal with the growing state space, we introduce \texttt{CU-LB} (Algorithm~\ref{alg:LB-CBF-CU}) and \texttt{CU-UB} (Algorithm~\ref{alg:UB-CBF-CU}); two variants of \texttt{CMS-CU} where the \emph{counters gap}, i.e., the difference between the values of the maximal and minimal counter, is capped by a constant $g\in\mathbb{N}$.  

The approximation error of the constructed capped variants \texttt{CMS-CU} bounds the approximation error of  \texttt{CMS-CU} with a high probability, as shown in Theorem~\ref{th:mainHPConcentration}. In these two variants of \texttt{CMS-CU}, the counters gap is capped. Therefore, there dynamic can be modeled as discrete-time Markov chain with finite state space. 

In the reminder of this section, we provide details on the construction of \texttt{CU-LB} and \texttt{CU-UB}, and we  


\begin{algorithm}[t]
\caption{\texttt{LB-CU}}
\begin{algorithmic}[1]
\State \textbf{Input:} $(S_t)_{t\in \aIntInterval{T}}$, $g$
\State  $\LBCBFCU{g}{0} \gets \mathbf{0}$
\For{$t$ in $\aIntInterval{T}$}
    \If{$\LBCBFCUElement{g}{\text{max}}{t-1}-\LBCBFCUElement{g}{\text{min}}{t-1} = g$, and $\min_{i\in S_t} \LBCBFCUElement{g}{i}{t-1}=\LBCBFCUElement{g}{\text{max}}{t-1}$}
        \State $\LBCBFCU{g}{t} \gets \LBCBFCU{g}{t-1}$ \label{line:LBNoUpdate}
    \Else
        \State $\LBCBFCU{g}{t} \gets$ \text{CU}$\left(\LBCBFCU{g}{t-1}, S_t\right)$ \label{line:LBCuUpdate}
    \EndIf
\EndFor
\end{algorithmic}
\label{alg:LB-CBF-CU}
\end{algorithm}

A key idea to prove Theorems~\ref{th:main} and~\ref{th:mainHPConcentration}, is to introduce two variants OF \texttt{CMS-CU}, which we call \texttt{LB-CU} and \texttt{UB-CU}. The dynamics of \texttt{LB-CU} and \texttt{UB-CU} are outlined in Algorithms~\ref{alg:LB-CBF-CU} and~\ref{alg:UB-CBF-CU}, respectively. Both variants feature a parameter~$g\in \mathbb{N}$. 
In \texttt{LB-CU}, we denote the counter values at step~$t$ as~$\LBCBFCU{g}{t}= (\LBCBFCUElement{g}{j}{t})_{j\in \aIntInterval{M}}$, and we denote the maximum and minimum counter values, namely~$\max_{j\in \aIntInterval{M}} \LBCBFCUElement{g}{j}{t}$ and~$\min_{j\in \aIntInterval{M}} \LBCBFCUElement{g}{j}{t}$, as~$\LBCBFCUElement{g}{\max}{t}$ and~$\LBCBFCUElement{g}{\min}{t}$, respectively.
We use a similar notation for \texttt{UB-CU}, by replacing the superscript ``$\text{lb}$'' with ``$\text{ub}$''.
Initially, all counters are equal to~$0$. At each step~$t\geq 1$,~$S_t=\{h_l(r_t):\; l\in \aIntInterval{d}\}$ represents the~$d$ selected counters. Both \texttt{LB-CU} and \texttt{UB-CU} update counter values based on the previous state, distinguishing between two cases:
  \begin{enumerate}
    \item If the gap between maximum and minimum counter values equals $g$, and all selected counters have values equal to the maximum counter value, \texttt{LB-CU} performs no updates (line~\ref{line:LBNoUpdate}), while in \texttt{UB-CU}, counters with values equal to $\UBCBFCUElement{g}{\text{min}}{t-1}$ are incremented (line~\ref{line:UbMinUpdate}), along with the selected counters (line~\ref{line:UbCuUpdate}).
    \item Otherwise, \texttt{LB-CU} and \texttt{UB-CU} update the counters according to the conservative update in~\eqref{e:DynamicsCU} (lines~\ref{line:LBCuUpdate} and~\ref{line:UbCuUpdate}). 
\end{enumerate}
Observe that for any stream of length~$T$ and any value $g\geq T$, \texttt{LB-CU}, \texttt{UB-CU}, and \texttt{CU} produce identical counter vectors, i.e., $\LBCBFCU{g}{t}=\UBCBFCU{g}{t}=\CBFCU{t}$, for any $t\in \aIntInterval{T}$. Similarly to~$e^{*}(t)$ in CU, we define~$\LBErrorstar{g}{t}$ and~$\UBErrorstar{g}{t}$ as errors with probability distributions identical to the error for any item~$i$ with~$n_{i}(t)=0$, in \texttt{LB-CU} and \texttt{UB-CU}, respectively.

Efficient computation of both quantities relies on similar techniques. Therefore, we first introduce a method to compute~$\E{\LBErrorstar{g}{T}}/T$ and subsequently demonstrate how to adapt this method to calculate~$\E{\UBErrorstar{g}{T}}/T$. A key point of our method is to study the stochastic evolution of the number of counters that are far from the minimum value counter by any value~$l$, denoted~$\LBExcessEle{g}{l}(t)$. Formally,
\begin{align}\label{e:defExcessLBCU}
        \LBExcessEle{g}{l}(t) \triangleq \sum_{j=1}^{M} \mathds{1}\left( \LBCBFCUElement{g}{j}{t} - \LBCBFCUElement{g}{\min}{t} =l   \right).
\end{align}
Indeed, $(\LBExcess{g}(t)=( \LBExcessEle{g}{l}(t))_{l\in \mathbb{N}})_t$ is a time-homogeneous Markov chain with finite state space, denoted~$\Omega_g$. Moreover, the conditional expectation of~$\LBErrorstar{g}{t}-\LBErrorstar{g}{t-1}$ given~$(\LBExcess{g}(t), \LBExcess{g}(t-1)) = (\mathbf{k^{'}},\mathbf{k})$, is invariant with respect to~$t$, denoted as~$\LBProbaError{g}{k}{k^{'}}$.~Let $\LBMatrixError{g}$ be the matrix with components $\LBProbaError{g}{k}{k^{'}}$ for any $(\mathbf{k},\mathbf{k^{'}})\in (\Omega_g)^{2}$. $\LBMatrixTrans{g}$ denotes the one-step transition probabilities matrix of~$(\LBExcess{g}(t))_t$, $\LBOccupancyEle{g}{k}(t)$ represents the probability that $\LBExcess{g}(t)=\mathbf{k}$, and $\LBOccupancy{g}(t)$ is the vector of these probabilities for each state $\mathbf{k}\in \Omega_g$.

\begin{proposition}\label{prop:EfficientComputation}
The quantity~$\E{\LBErrorstar{g}{T}}$ satisfies, 
\begin{align}\label{e:ExpErrorLBg}
            \E{\LBErrorstar{g}{T}} = \left\langle  \sum_{t=0}^{T-1}\LBOccupancy{g}(t) ,  \LBMatrixTrans{g} \odot \LBMatrixError{g} \cdot \mathbf{1}^\intercal \right\rangle,
\end{align}
where~$\odot$ is the element-wise product, and~$\mathbf{1}^{\intercal}$ represents a column vector with $|\Omega_g|$ rows, where each entry is equal to~$1$. Furthermore, computing~$\E{\LBErrorstar{g}{T}}$ using~\eqref{e:ExpErrorLBg} incurs a time complexity of~$\mathcal{O}\left(\max(d,T) M \binom{M+g-d}{g}\right)$.
\end{proposition}   

\begin{proposition}\label{prop:HPConcentration}
    The random variable~$\LBErrorstar{g}{T}/T$ converges almost surely to constants as~$T$ tends to infinity. Formally, 

        \begin{align}
            \Proba{\lim_{T\to +\infty} \LBErrorstar{g}{T}/ T  = \left\langle  \LBOccupancy{g}(\infty) ,  \LBMatrixTrans{g} \odot \LBMatrixError{g} \cdot \mathbf{1}^\intercal \right\rangle} = 1, 
        \end{align}
where $\LBOccupancy{g}(\infty)$ is the limiting distribution of~$(\LBExcess{g}(t))_t$. 
\end{proposition}


\begin{algorithm}[t]
\caption{\texttt{UB-CU}}
\begin{algorithmic}[1]
\State \textbf{Input:} $(S_t)_{t\in \aIntInterval{T}}$, $g$
\State $\UBCBFCU{g}{0}  \gets \mathbf{0}$
\For{$t$ in $\aIntInterval{T}$}
    \State $\UBCBFCU{g}{t} \gets$ \text{CU}$\left(\UBCBFCU{g}{t-1}, S_t\right)$ \label{line:UbCuUpdate}
     \If{$\UBCBFCUElement{g}{\text{max}}{t-1}-\UBCBFCUElement{g}{\text{min}}{t-1} = g$, and $\min_{i\in S_t} \UBCBFCUElement{g}{i}{t-1}=\UBCBFCUElement{g}{\text{max}}{t-1}$}
        \State $\UBCBFCUElement{g}{j}{t}= \UBCBFCUElement{g}{j}{t-1} + 1, \; \forall j\in \aIntInterval{M}: \; \UBCBFCUElement{g}{j}{t-1}= \UBCBFCUElement{g}{\text{min}}{t-1}$\label{line:UbMinUpdate}
    \EndIf
\EndFor
\end{algorithmic}
\label{alg:UB-CBF-CU}
\end{algorithm}

\begin{theorem}\label{th:main}
    Under Assumption~\ref{assum:UniformCounters}, for any~$g\in \mathbb{N}$, there exist positive values~$\ell_g(T)$ and~$U_g(T)$, such that the error~$e^{*}(T)$ satisfies,
\begin{align}
 \ell_{g}(T)   \leq   \E{e^{*}(T)/T} \leq U_{g}(T),
\end{align}
where~$(\ell_{g}(T))_g$ and~$(U_{g}(T))_g$ form strictly increasing and decreasing sequences for~$g<T$, respectively. Conversely, $\ell_g(T)=U_g(T)$ when~$g\geq T$. Furthermore, these quantities~$\ell_{g}(T)$ and~$U_{g}(T)$ can be computed with time complexity~$\mathcal{O}(\max(d,T) M\binom{M+g-d}{g})$. 

\end{theorem}

\begin{theorem}\label{th:mainHPConcentration}
Under Assumption~\ref{assum:UniformCounters}, for any~$g\in\mathbb{N}$, the error $e^{*}(T)$ satisfies, 
    \begin{align}
\lim_{T \to +\infty} \Proba{\ell_{g}(\infty)   \leq   e^{*}(T)/T \leq U_{g}(\infty)} = 1,
\end{align}
where~$\ell_{g}(\infty) = \lim_{T\to \infty} \ell_g(T)$ and~$U_{g}(\infty) = \lim_{T\to \infty} U_g(T)$. 
\end{theorem}

Theorem~\ref{th:mainHPConcentration} proves that~$e^{*}(T)/T$ concentrates around the interval~$[l_{g}(\infty), U_{g}(\infty)]$ for large values of~$T$. The values~$l_{g}(\infty)$ and~$U_{g}(\infty)$ can be approximated by the values of the sequences $l_{g}(T)$ and $U_{g}(T)$ for large values of~$T$. 


 


\begin{proposition}\label{prop:SandwichBound}
For any~$g\in \mathbb{N}$ and any sequence of selected counters~$(S_t)$, the error~$e^{*}(T)$ satisfies, 
    \begin{equation}\label{e:SandwichError}
       \LBErrorstar{g}{T}     \leq   e^{*}(T) \leq \UBErrorstar{g}{T}.
    \end{equation} 
Additionally, the sequences~$(\E{\LBErrorstar{g}{T}}/T)_g$ and~$(\E{\UBErrorstar{g}{t}}/T)_g$ are strictly increasing and decreasing sequences for~$g<T$, respectively. On the other hand, for any~$g\geq T$, both sequences converge to~$\E{e^{*}(T)/T}$. 
\end{proposition}   

Proposition~\ref{prop:SandwichBound} proves the first part of Theorem~\ref{th:main}, where~$\ell_g(T)$ and~$U_{g}(T)$ denote $\E{\LBErrorstar{g}{T}}/T$ and~$\E{\UBErrorstar{g}{T}}/T$ respectively. 

The proof of Theorem~\ref{th:main} readily follows from Propositions~\ref{prop:SandwichBound} and~\ref{prop:EfficientComputation}, while establishing Theorem~\ref{th:mainHPConcentration} is straightforward with Propositions~\ref{prop:SandwichBound} and~\ref{prop:HPConcentration}.


==> main_results/error_computation_22April.tex <==



One direct approach to study~$\CMSCU$ under Assumption~\ref{assum:UniformCounters} is to recognize that~$(\mathbf{Y}(t))_t$ forms a discrete-time Markov chain, allowing for the computation of the probability that~$\mathbf{Y}(t)$ is in a specific state. However, the state space of this Markov chain grows fast with~$t$. To manage the growing state space, we introduce $\LBCU$ (Algorithm~\ref{alg:LB-CBF-CU}) and $\UBCU$ 
(Algorithm~\ref{alg:UB-CBF-CU}), two variants of $\CMSCU$ in which the difference between the highest and lowest counter values, referred to as the \emph{counters gap}, is capped by a constant~$g\in\mathbb{N}$.   

% To manage this expanding state space, we introduce CU-LB (Algorithm~\ref{alg:LB-CBF-CU}) and CU-UB (Algorithm~\ref{alg:UB-CBF-CU}), two variants of CMS-CU that limit the difference between the highest and lowest counter values (the counters gap) to a constant $g \in \mathbb{N}$.


% Theorem~\ref{th:main} introduces $\ell_{g}(T)$ and $U_g(T)$, which corresponds to the expected average estimation errors of the capped variants $\LBCU$ and $\UBCU$. Property~\ref{eq:stationary} shows that 

As shown in Theorem~\ref{th:main}, the expected average estimation errors~$\ell_g(T)$ and~$U_g(T)$ of the capped variants $\LBCU$ and $\UBCU$ match the expected average estimation error of $\CMSCU$ ($\E{\nicefrac{e^{*}(T)}{T}}$) when $g \geq T$ (Property~\ref{eq:stationary}). When $g < T$, $\E{\nicefrac{e^{*}(T)}{T}}$ is bounded by these two sequences (Property~\ref{eq:sandwich_expectation}). Additionally, as $T\to\infty$, the value~$\nicefrac{e^{*}(T)}{T}$ concentrates in the interval~$[\ell_{g}(\infty), U_{g}(\infty)]$ with high probability (Property~\ref{eq:sandwich_proba}). 
% almost surely (Property~\ref{eq:sandwich_proba}).

% Due to the capped counters gap in the two $\CMSCU$ variants, the process can be modeled as a discrete-time Markov chain with a finite state space. This allows for efficient computation of the estimation error of \texttt{CU-LB} and \texttt{CU-UB} with a time complexity of  \( \mathcal{O}(\max(d, T) \cdot m \cdot \binom{m + g - d}{g}) \) (Property~\ref{eq:complexity}).


Due to the capped counters gap in the two~$\CMSCU$ variants, one could analyze the estimation error by studying a discrete-time Markov chain with finite state space. This allows for efficient computation of the estimation error of~$\LBCU$ and~$\UBCU$ with a time complexity of~\( \mathcal{O}(\max(d, T) \cdot m \cdot \binom{m + g - d}{g}) \) (Property~\ref{eq:complexity}). 

% A key point of our method is to study the stochastic evolution of the number of counters that are far from the minimum value counter by any value~$l$, denoted~$\LBExcessEle{g}{l}(t)$. Formally,
% \begin{align}\label{e:defExcessLBCU}
%         \LBExcessEle{g}{l}(t) \triangleq \sum_{j=1}^{M} \mathds{1}\left( \LBCBFCUElement{g}{j}{t} - \LBCBFCUElement{g}{\min}{t} =l   \right).
% \end{align}
% Indeed, $(\LBExcess{g}(t)=( \LBExcessEle{g}{l}(t))_{l\in \mathbb{N}})_t$ is a time-homogeneous Markov chain with finite state space, denoted~$\Omega_g$.




\begin{theorem}\label{th:main}
    Under Assumption~\ref{assum:UniformCounters}, there exist a non-decreasing sequence~$(\ell_g(T))_g$ and a non-increasing sequence $(U_g(T))_g$ with limits $\ell_g(\infty)$ and $U_g(\infty)$, respectively. These sequences satisfy the following properties:
    \begin{enumerate}
        \item When \( g \geq T \), \( \ell_g(T) = \E{\nicefrac{e^{*}(T)}{T}} = U_g(T) \). \label{eq:stationary}
        \item For \( g < T \), the expected value is bounded: \( \ell_{g}(T)  \leq \E{\nicefrac{e^{*}(T)}{T}} \leq U_{g}(T) \). \label{eq:sandwich_expectation}
        \item As \( T \to \infty \), the probability of \( \ell_g(\infty) \leq e^{*}(T)/T \leq U_g(\infty) \) converges to 1. \label{eq:sandwich_proba}
        \item The sequences \( \ell_g(T) \) and \( U_g(T) \) can be computed with a time complexity of \( \mathcal{O}(\max(d, T)\cdot m \cdot \binom{m + g - d}{g}) \). \label{eq:complexity}
        
    \end{enumerate}
\end{theorem}

This section is organized as follows; first, we describe the construction of $\LBCU$ and $\UBCU$ in Section~\ref{sec:capped_sketch}. Second, in Section~\ref{sec:capped_approximation_errors}, we analyze their approximation errors and prove Properties~\ref{eq:stationary} and \ref{eq:sandwich_expectation}.  Third, in Section~\ref{sec:efficient_computation}, we leverage the fact that $\LBCU$ and $\UBCU$ can be modeled as discrete-time Markov chains with finite state spaces to efficiently compute their estimation errors, proving Properties~\ref{eq:complexity} and~\ref{eq:sandwich_proba}. Finally, in Section~\ref{sec:case_study}, we provide closed form expressions of $\ell_g(T)$ and $U_g(T)$ in two particular use-cases; $d=m-1$, and $g=1$.

\subsubsection{The Construction of the Counters Gap Capped \texttt{CMS-CU}}
\label{sec:capped_sketch}
% \input{estimation_errror/capped_sketch}
\begin{algorithm}[t]
\caption{$\LBCU$}
\begin{algorithmic}[1]
\State \textbf{Input:} $(r_t)_{t\in \aIntInterval{T}}$, $g$
\State  $\LBCBFCU{g}{0} \gets \mathbf{0}$
\For{$t$ in $\aIntInterval{T}$}
    \If{$\LBCBFCUElement{g}{\text{max}}{t-1}-\LBCBFCUElement{g}{\text{min}}{t-1} = g$, and $\min_{u\in \bm{h}(r_t)} \LBCBFCUElement{g}{u}{t-1}=\LBCBFCUElement{g}{\text{max}}{t-1}$}
        \State $\LBCBFCU{g}{t} \gets \LBCBFCU{g}{t-1}$ \label{line:LBNoUpdate}
    \Else
        \State $\LBCBFCU{g}{t} \gets$ \text{CU}$\left(\LBCBFCU{g}{t-1}, \bm{h}(r_t)\right)$ \label{line:LBCuUpdate}
    \EndIf
\EndFor
\end{algorithmic}
\label{alg:LB-CBF-CU}
\end{algorithm}


\begin{algorithm}[t]
\caption{$\UBCU$}
\begin{algorithmic}[1]
\State \textbf{Input:} $(r_t)_{t\in \aIntInterval{T}}$, $g$
\State $\UBCBFCU{g}{0}  \gets \mathbf{0}$
\For{$t$ in $\aIntInterval{T}$}
    \State $\UBCBFCU{g}{t} \gets$ \text{CU}$\left(\UBCBFCU{g}{t-1}, \bm{h}(r_t)\right)$ \label{line:UbCuUpdate}
     \If{$\UBCBFCUElement{g}{\text{max}}{t-1}-\UBCBFCUElement{g}{\text{min}}{t-1} = g$, and $\min_{u\in \bm{h}(r_t)} \UBCBFCUElement{g}{u}{t-1}=\UBCBFCUElement{g}{\text{max}}{t-1}$}
        \State $\UBCBFCUElement{g}{c}{t}= \UBCBFCUElement{g}{c}{t-1} + 1, \; \forall c\in \aIntInterval{m}: \; \UBCBFCUElement{g}{c}{t-1}= \UBCBFCUElement{g}{\text{min}}{t-1}$\label{line:UbMinUpdate}
    \EndIf
\EndFor
\end{algorithmic}
\label{alg:UB-CBF-CU}
\end{algorithm}


The key idea to prove Theorem~\ref{th:main} is to introduce two variants of $\CMSCU$, which we call $\LBCU$ and $\UBCU$. Their dynamics are outlined in Algorithms~\ref{alg:LB-CBF-CU} and~\ref{alg:UB-CBF-CU}. 
% The dynamics of $\LBCU$ and $\UBCU$ are outlined in Algorithms~\ref{alg:LB-CBF-CU} and~\ref{alg:UB-CBF-CU}, respectively.
Both variants feature a parameter~$g\in \mathbb{N}$. 
In \texttt{LB-CU}, we denote the counter values at step~$t$ as~$\LBCBFCU{g}{t}= (\LBCBFCUElement{g}{c}{t})_{c\in \aIntInterval{m}}$, and we denote the maximum and minimum counter values, namely~$\max_{c\in \aIntInterval{m}} \LBCBFCUElement{g}{c}{t}$ and~$\min_{c\in \aIntInterval{m}} \LBCBFCUElement{g}{c}{t}$, as~$\LBCBFCUElement{g}{\max}{t}$ and~$\LBCBFCUElement{g}{\min}{t}$, respectively.
We use a similar notation for $\UBCU$, by replacing the superscript ``$\text{lb}$'' with ``$\text{ub}$''.
Initially, all counters are equal to~$0$. At each step~$t\geq 1$, both $\LBCU$ and $\UBCU$ update counter values based on the previous state, distinguishing between two cases:
  \begin{enumerate}
    \item If the gap between maximum and minimum counter values equals~$g$, and all selected counters have values equal to the maximum counter value, $\LBCU$ performs no updates (line~\ref{line:LBNoUpdate}), while in $\UBCU$, counters with values equal to $\UBCBFCUElement{g}{\text{min}}{t-1}$ are incremented (line~\ref{line:UbMinUpdate}), along with the selected counters (line~\ref{line:UbCuUpdate}).
    \item Otherwise, $\LBCU$ and $\UBCU$ update the counters according to the conservative update in~\eqref{e:DynamicsCU} (lines~\ref{line:LBCuUpdate} and~\ref{line:UbCuUpdate}). 
\end{enumerate}

Similarly to~$e^{*}(t)$ in $\CMSCU$, we define~$\LBErrorstar{g}{t}$ and~$\UBErrorstar{g}{t}$ as errors with probability distributions identical to the errors for any item~$i$ with~$n_{i}(t)=0$, in $\LBCU$ and~$\UBCU$, respectively. We use $\ell_g(T)$ and~$U_{g}(T)$ to denote $\E{\LBErrorstar{g}{T}}/T$ and~$\E{\UBErrorstar{g}{T}}/T$ respectively.

\subsubsection{The Estimation Error of the Counters Gap Capped \texttt{CMS-CU}}
\label{sec:capped_approximation_errors}

Before delving into the analysis of the estimation errors of $\LBCU$ and $\UBCU$, we make the following observations about these two processes:
\begin{enumerate}
    \item The gap between the maximum and minimum counter values in both $\LBCU$ and $\UBCU$ with the same parameter~$g$ is at most~$g$. \label{obs:cap}
    \item For any stream of length~$T$ and any value $g\geq T$, $\LBCU$, $\UBCU$, and $\CMSCU$ produce identical counter vectors, i.e., $\LBCBFCU{g}{t}=\UBCBFCU{g}{t}=\CBFCU{t}$, for any $t\in \aIntInterval{T}$.\label{obs:stationnary}
\end{enumerate}
Both Observation~\ref{obs:cap} and Observation~\ref{obs:stationnary} follows from the construction of \texttt{LB-CU} and \texttt{UB-CU}, and can be formally proven by a simple recursion on $T$.   

Property~\ref{eq:stationary} is an immediate result Observation~\ref{obs:stationnary}. While Property~\ref{eq:sandwich_expectation} follows from Observation~\ref{obs:cap} through Lemma~\ref{lem:monotony} (Proof in Section~\ref{proof:monothony}).
\begin{lemma}
    \label{lem:monotony}
    For any stream $(r_t)_{t\geq0}$, $(\LBCBFCU{g}{t})_{g\geq 0}$ (resp. $(\UBCBFCU{g}{t})_{g\geq 0}$) is an element-wise non-decreasing (resp. non-increasing) sequence. 
\end{lemma}
Lemma~\ref{lem:monotony} implies that~$ \LBCBFCU{g}{T} \leq \CBFCU{T} \leq \UBCBFCU{g}{T}$ for any~$g\in \mathbb{N}$. In particular, this inequality is valid for the errors of the items that did not appear in the stream before time~$T$, proving Property~\ref{eq:sandwich_expectation}.

Moreover, for any~$g<T$, it is easy to find a sequence~$(S_t)_{t\geq 0}$ of selected counters such that~$\LBErrorstar{g}{T} < \LBErrorstar{g+1}{T}$ and~$\UBErrorstar{g+1}{T} < \UBErrorstar{g}{T}$, thus~$\E{\LBErrorstar{g}{T}} < \E{\LBErrorstar{g+1}{T}}$ and $\E{\UBErrorstar{g+1}{T}} < \E{\UBErrorstar{g}{T}}$. It follows that the sequences~$(\ell_g(T))_g$ (resp.~$(U_g(T))_g$) is a non-decreasing (resp. non-decreasing) sequence. 

\subsubsection{Efficient Computation of the Estimation Error of the Counters Gap Capped \texttt{CMS-CU}}
\label{sec:efficient_computation}

Efficient computation of both quantities relies on similar techniques. Therefore, we first introduce a method to compute~$\E{\LBErrorstar{g}{T}}/T$ and subsequently demonstrate how to adapt this method to calculate~$\E{\UBErrorstar{g}{T}}/T$. A key point of our method is to study the stochastic evolution of the number of counters that are far from the minimum value counter by any value~$l$, denoted~$\LBExcessEle{g}{l}(t)$. Formally,
\begin{align}\label{e:defExcessLBCU}
        \LBExcessEle{g}{l}(t) \triangleq \sum_{j=1}^{M} \mathds{1}\left( \LBCBFCUElement{g}{j}{t} - \LBCBFCUElement{g}{\min}{t} =l   \right).
\end{align}
Indeed, $(\LBExcess{g}(t)=( \LBExcessEle{g}{l}(t))_{l\in \mathbb{N}})_t$ is a time-homogeneous Markov chain with finite state space, denoted~$\Omega_g$. Moreover, the conditional expectation of~$\LBErrorstar{g}{t}-\LBErrorstar{g}{t-1}$ given~$(\LBExcess{g}(t), \LBExcess{g}(t-1)) = (\mathbf{k^{'}},\mathbf{k})$, is invariant with respect to~$t$, denoted as~$\LBProbaError{g}{k}{k^{'}}$.~Let $\LBMatrixError{g}$ be the matrix with components $\LBProbaError{g}{k}{k^{'}}$ for any $(\mathbf{k},\mathbf{k^{'}})\in (\Omega_g)^{2}$. $\LBMatrixTrans{g}$ denotes the one-step transition probabilities matrix of~$(\LBExcess{g}(t))_t$, $\LBOccupancyEle{g}{k}(t)$ represents the probability that $\LBExcess{g}(t)=\mathbf{k}$, and $\LBOccupancy{g}(t)$ is the vector of these probabilities for each state $\mathbf{k}\in \Omega_g$.

\begin{proposition}\label{prop:EfficientComputation}
The quantity~$\E{\LBErrorstar{g}{T}}$ satisfies, 
\begin{align}\label{e:ExpErrorLBg}
            \E{\LBErrorstar{g}{T}} = \left\langle  \sum_{t=0}^{T-1}\LBOccupancy{g}(t) ,  \LBMatrixTrans{g} \odot \LBMatrixError{g} \cdot \mathbf{1}^\intercal \right\rangle,
\end{align}
where~$\odot$ is the element-wise product, and~$\mathbf{1}^{\intercal}$ represents a column vector with $|\Omega_g|$ rows, where each entry is equal to~$1$. Furthermore, computing~$\E{\LBErrorstar{g}{T}}$ using~\eqref{e:ExpErrorLBg} incurs a time complexity of~$\mathcal{O}\left(\max(d,T) m \binom{m+g-d}{g}\right)$.
\end{proposition}  

\begin{proposition}\label{prop:HPConcentration}
    The random variable~$\LBErrorstar{g}{T}/T$ converges almost surely to constants as~$T$ tends to infinity. Formally, 
        \begin{align}
            \Proba{\lim_{T\to +\infty} \LBErrorstar{g}{T}/ T  = \left\langle  \LBOccupancy{g}(\infty) ,  \LBMatrixTrans{g} \odot \LBMatrixError{g} \cdot \mathbf{1}^\intercal \right\rangle} = 1, 
        \end{align}
where $\LBOccupancy{g}(\infty)$ is the limiting distribution of~$(\LBExcess{g}(t))_t$. 
\end{proposition}




% \begin{proposition}\label{prop:SandwichBound}
% For any~$g\in \mathbb{N}$ and any sequence of selected counters~$(S_t)$, the error~$e^{*}(T)$ satisfies, $\LBErrorstar{g}{T}     \leq   e^{*}(T) \leq \UBErrorstar{g}{T}$. Additionally, the sequences~$(\E{\LBErrorstar{g}{T}}/T)_g$ and~$(\E{\UBErrorstar{g}{t}}/T)_g$ are strictly increasing and decreasing sequences for~$g<T$, respectively. On the other hand, for any~$g\geq T$, both sequences converge to~$\E{e^{*}(T)/T}$. 
% \end{proposition}   

% Proposition~\ref{prop:SandwichBound} proves the first part of Theorem~\ref{th:main}, where~$\ell_g(T)$ and~$U_{g}(T)$ denote $\E{\LBErrorstar{g}{T}}/T$ and~$\E{\UBErrorstar{g}{T}}/T$ respectively. 

\subsection{Case Study}
\label{sec:case_study}


\begin{proposition}
    \begin{align}
        e^{*}(T) \leq    \LBErrorstar{g}{T} + \sum_{t=1}^{T} \mathds{1}(G(t) > g)  
    \end{align}
\end{proposition}



==> main_results/motivation_3Mai.tex <==
In the introduction, we highlighted experimental findings from prior research~\cite{bianchi2012modelingCMSCU,MAZZIANE2022CMSCU,FusyExpCMSCU2023} concerning the error in~$\CMSCU$, demonstrating two key points. First, infrequent items exhibit greater errors compared to others. 
% and provides empirical evidence that the approximation error under this assumption acts as an upper bound for skewed distributions
Second, infrequent items' errors seem maximal when~$d$ distinct counters are uniformly selected at random within $\CMSCU$~\cite{bianchi2012modelingCMSCU}. This particular instance of $\CMSCU$ is formalized in~Assumption~\ref{assum:UniformCounters} and can be interpreted as the fusion of Assumptions~\ref{assum:IdealHash} and~\ref{assum:DistinctRequests}.
% Driven by these empirical observations, our work focuses on the error for infrequent items in $\CMSCU$ under the uniform counters selection setting, formalized in Assumption~\ref{assum:UniformCounters}.
% . This configuration arises when Assumption~\ref{assum:UniformCounters} holds.
\begin{assumption}[Uniform Counters Selection]\label{assum:UniformCounters}
    The sets $(\bm{h}(r_t))_{t\in \mathbb{N}}$ are i.i.d. uniform random variables over $d$-sized subsets of $\aIntInterval{m}$, denoted as $\binom{\aIntInterval{m}}{d}$.
\end{assumption}
% The rest of Section~\ref{sec:estimation_error} is organized as follows. Section~\ref{sec:motivation} presents arguments supporting that $\CMSCU$ under Assumption~\ref{assum:UniformCounters} corresponds to the worst-case error scenario. Afterwards, Section~\ref{sec:capped_sketch} lays out our lower and upper bounds on the estimation error in the uniform counters selection regime. 
% Assumption~\ref{assum:UniformCounters} holds when Assumptions~\ref{assum:DistinctRequests} and~\ref{assum:IdealHash} are satisfied. 

% can be interpreted as the fusion of Assumptions~\ref{assum:DistinctRequests} and A. The first one, described in Assumption~\ref{assum:IdealHash}, supposes that hash functions map items uniformly and independently over~$\binom{\aIntInterval{m}}{d}$. The second condition, presented in Assumption~\ref{assum:DistinctRequests}, considers a specific type of stream where each item appears at most once.   


 %We observe that 

 We argue that the particular instance of $\CMSCU$ in which counters are uniformly selected is relevant to deriving general bounds on the error applicable for any stream. To formalize this claim, we interpret Assumption~\ref{assum:UniformCounters} as the fusion of two conditions.



 
 % is met when considering a specific stream $\bm{r}=(r_t)_{t\in \aIntInterval{T}}$,  provided that hash functions map items uniformly and independently over~$\binom{\aIntInterval{m}}{d}$. This property is formalized in Assumptions~\ref{assum:IdealHash} and~\ref{assum:DistinctRequests}. 
 
 
%  \begin{assumption}[Ideal Hash Function Model]\label{assum:IdealHash}
%         The sets~$\left( \bm{h}(i)\right)_{i\in \mathcal{I}}$ are i.i.d. uniform random variables over~$\binom{\aIntInterval{m}}{d}$.
% \end{assumption}
%  \begin{assumption}\label{assum:DistinctRequests}
%     The stream~$\mathbf{r}$ consists of distinct items, i.e.,~$r_t\neq r_s$ for every~$t\neq s\in \aIntInterval{T}$.
% \end{assumption}

Many works adopt ideal hashing models despite the impractical computational cost of their design~\cite{BroderBloomFilter2003,bianchi2012modelingCMSCU,GILBloomCMSCU,fusy2023phase}. Remarkably, these models often predict the performance of algorithms operating with practical hash functions of weaker notions of independence. A~theoretical rationale for this phenomenon is elucidated in~\cite{mitzenmacher2008simple}.  



% Despite the impractical computational cost of designing ideal hash functions, many works adopt similar hashing models~\cite{BroderBloomFilter2003,bianchi2012modelingCMSCU,GILBloomCMSCU,fusy2023phase}.
% Provided that the hash functions are ideal, $\CMSCU$ on a particular stream where each item appears at most once coincides with the uniform counters selection variant of $\CMSCU$. 

Assumption~\ref{assum:DistinctRequests} deviates from typical data stream models. For example, previous studies of $\CMSCU$~\cite{GILBloomCMSCU,MAZZIANE2022CMSCU,fusy2023phase} assume a random stationary stream and provide probabilistic bounds on the error in terms of items' probabilities of appearance. However, these bounds fall short in capturing the benefits of \textit{conservative updates} when items' probabilities are small. One could perceive a stream conforming to Assumption~\ref{assum:DistinctRequests} as a highly probable realization of a stochastic process where all items' probabilities are equal, and the catalog of items is infinite w.r.t. the stream length, i.e., $T \ll |\mathcal{I}|$. This perspective highlights streams following Assumption~\ref{assum:DistinctRequests} as scenarios where existing bounds fail to capture the advantages of~$\CMSCU$.




 








% Nonetheless, generic error bounds applicable for any stream are absent for~$\CMSCU$.  






We conjecture that the expected estimation error for items in $\CMSCU$ reaches its maximum when the stream adheres to Assumption~\ref{assum:DistinctRequests}. To state this conjecture precisely, we introduce additional notation.

% We employ the symbols~$e_{i}(t,\bm{r})$ and~$n_{i}(t,\bm{r})$ to signify the error and the count for an item~$i$ in the specific stream $\mathbf{r}$ at step~$t$, respectively. Under Assumption~\ref{assum:IdealHash}, for any two items~$i, j\in\mathcal{I}$ and any stream $\bm{r}$ such that $n_{i}(t,\bm{r})=0$ and $n_{j}(t,\bm{r})=0$, the errors~$e_{i}(t,\bm{r})$ and~$e_{j}(t,\bm{r})$ are identically distributed. Let~$e^{*}(t,\bm{r})$ denote a random variable following their common probability distribution. Furthermore, for any two streams $\bm{r}$ and $\bm{a}$ satisfying Assumption~\ref{assum:DistinctRequests}, $e^{*}(t,\bm{a})$ and $e^{*}(t,\bm{r})$ share identical probability distribution and we define $e^{*}(t)$ as a random variable with that distribution. 

\begin{conjecture}\label{conj:maximalError}
Under Assumption~\ref{assum:IdealHash}, for any item $i$ and stream $\bm{r}$, the following inequality holds: $\E{e_{i}(t,\bm{r})} \leq \E{e^{*}(t)}$.
\end{conjecture}
% While Assumption~\ref{assum:DistinctRequests} does not usually hold, it serves in upper-bounding the estimation error, as shown in Proposition~\ref{prop:WorstErrorItemNotReq}.
To support Conjecture~\ref{conj:maximalError}, Proposition~\ref{prop:WorstErrorItemNotReq} formally proves that for any stream, the maximal expected estimation error occurs for items with the lowest count. 

\begin{proposition}\label{prop:WorstErrorItemNotReq}
    Under Assumption~\ref{assum:IdealHash}, for any item~$i$ and stream~$\bm{r}$, the following inequality holds: $\E{e_{i}(t,\bm{r})} \leq \E{e^{*}(t,\bm{r})}$.
    % where the expectation is taken over the random choice of the hash functions. 
\end{proposition}
 Proposition~\ref{prop:WorstErrorItemNotReq} (proof in Appendix~\ref{proof:propositionWorstErrorItem}) partially validates the empirical observation that the expected error of an item~$i$ at time~$t$ in $\CMSCU$ tends to increase as~$n_{i}(t)$ decreases~\cite{bianchi2012modelingCMSCU,MAZZIANE2022CMSCU}. Notably, Bianchi et al.~\cite{bianchi2012modelingCMSCU} experimentally observed that frequent items have negligible errors, whereas infrequent ones are estimated with the same value, called \emph{error floor}, which corresponds to $\E{e^{*}(\bm{r}, t)}$ in our context. Proposition~\ref{prop:WorstErrorItemNotReq} and the simulations in~\cite{bianchi2012modelingCMSCU}, suggesting that $\E{e^{*}(\bm{r},t)}\leq \E{e^{*}(t)}$, bolster the plausibility of Conjecture~\ref{conj:maximalError}. The remainder of this paper focuses on computing $\nicefrac{e^{*}(T)}{T}$ for $T>0$, which we refer to as the average estimation error of~$\CMSCU$. We are interested in both the asymptotic properties of this error and its finite-time properties. 

 % We are both interested in the asymptotic properties of this estimation error, as well as in it is finite distance properties. 

 
 % Simulations in~\cite{bianchi2012modelingCMSCU} suggest that $\E{e^{*}(\bm{r},t)}\leq \E{e^{*}(t)}$, which combined with Proposition~\ref{prop:WorstErrorItemNotReq}, aligns with Conjecture~\ref{conj:maximalError}. 
 
 % One could prove Conjecture~\ref{conj:maximalError} 
 
 
 % They also observed that the \emph{error floor} is maximal under the uniform counters selection assumption, which combined with Proposition~\ref{prop:WorstErrorItemNotReq} aligns with Conjecture~\ref{conj:maximalError}. 
 


 % is the \emph{error floor}.  Furthermore, it was observed that the \emph{error floor} is maximal under the uniform counters selection assumption, in this setting, it corresponds to $\E{e^{*}(t)}$. 


%  However, we conjecture that this particular stream represents a worst-case error stream for infrequent items, and therefore so is Assumption~\ref{assum:UniformCounters}. 

% with the lowest count, i.e., any item~$i$ such that~$n_{i}(t)=0$, is maximal for any stream satisfying Assumption~\ref{assum:DistinctRequests} in the ideal hash functions model. 


% The errors for an item $i$ in $\CMSCU$ are due to increments by other items $j$ such that $\bm{h}(i)\cap \bm{h}(j)\neq \emptyset$. The conservative update benefits the frequent items. Indeed for any two items $i$ and $j$ such that $n_{i}(t) \gg n_{j}(t)$, one would expect that if $c$ is a counter in $\bm{h}(i)$ and $u$ is a counter in $\bm{h}(j)$, then it is more likely that $Y_{c}(t) > Y_{u}(t)$. This explains why CMS-CU helps more frequent items than others. 


% Assumption~\ref{assum:DistinctRequests} considers a stream where all items are infrequent, i.e., $\forall i\in \mathcal{I}, \; n_{i}(t)\leq 1$. It is also the stream that minimizes $\max_{i\in \mathcal{I}} n_{i}(t)- \min_{j\in \mathcal{I}} n_{j}(t)$. Another interpretation for Assumption~\ref{assum:DistinctRequests} is that when the catalog of items is infinite w.r.t the time horizon, i.e., $T \ll |\mathcal{I}|$, it is unlikely that the same item would be requested more than once. All these interpretations support the uniform counter selection setting as a wors-case error setting

































 





